Smart Contract Vulnerabilities, Tools, and Benchmarks: an Updated Systematic Literature Review

Smart contracts are self-executing programs on blockchain platforms like Ethereum, which have revolutionized decentralized finance by enabling trustless transactions and the operation of decentralized applications. Despite their potential, the security of smart contracts remains a critical concern due to their immutability and transparency, which expose them to malicious actors. Numerous solutions for vulnerability detection have been proposed, but it is still unclear which one is the most effective. This paper presents a systematic literature review that explores vulnerabilities in Ethereum smart contracts, focusing on automated detection tools and benchmark evaluation. We reviewed 3,380 studies from five digital libraries and five major software engineering conferences, applying a structured selection process that resulted in 222 high-quality studies. The key results include a hierarchical taxonomy of 192 vulnerabilities grouped into 13 categories, a comprehensive list of 219 detection tools with corresponding functionalities, methods, and code transformation techniques, a mapping between our taxonomy and the list of tools, and a collection of 133 benchmarks used for tool evaluation. We conclude with a discussion about the insights into the current state of Ethereum smart contract security and directions for future research.

==> defs/author.tex <==
\author{Gerardo~Iuliano,
        Dario~Di~Nucci% <-this % stops a space
        \IEEEcompsocitemizethanks{\IEEEcompsocthanksitem G. Iuliano and D. Di Nucci are with the Software Engineering (SeSa) Lab, Department of Computer Science of the University of Salerno, Fisciano, Italy.\\
        \textbf{E-mails.} \{geiuliano, ddinucci\}@unisa.it}% <-this % stops an unwanted space
       %\thanks{Manuscript received April 19, 2005; revised August 26, 2015.}\protect\\
        % note need leading \protect in front of \\ to get a newline within \thanks as
        % \\ is fragile and will error, could use \hfil\break instead.    
}

==> defs/bibs.tex <==
\balance
\bibliographyA{bibs/appendix}
\bibliography{bibs/references}



==> defs/defs.tex <==
% RQ
\newcommand{\resquestion}[2]{ %
    \smallskip%
	\noindent\fcolorbox{black}{black!01}{%
		\parbox{0.99\linewidth}{% 
			\textbf{\textit{RQ$_{#1}$.}} \emph{#2} %
            }%
	}%
    \smallskip%
}%

% Take-Away
\newcommand{\finding}[2]{ %
    \smallskip%
	\noindent\fcolorbox{black}{blue!05}{%
		\parbox{0.98\linewidth}{% 
			\textbf{\faKey\ Take-Away \textbf{#1}.} #2 %
            }%
	}%
    \smallskip%
}%

% Revised text
\newcommand{\revised}[1]{
    \textcolor{blue}{#1}
}
% Revised text
\newcommand{\major}[1]{
    \textcolor{blue}{#1}
}

\newcommand{\myColor}[1]{
    \color{black}{#1}
}


% Put custom definitions here
\newcommand{\bluelink}[2]{\href{#1}{\textcolor{blue}{#2}}}

% geriRQ
\newcommand{\geriRQ}[2]{%
    \smallskip%
    \begin{mdframed}[hidealllines=true, backgroundcolor=gray!5]
        {\faSearch \hspace{0.2mm} \textbf{RQ\textsubscript{#1}.} \textit{#2}}
    \end{mdframed}
    \smallskip%
}

% geriBox
\newcommand{\geriBox}[1]{   
    \begin{mdframed}[hidealllines=true, backgroundcolor=gray!5]
        {\textit{#1}}
    \end{mdframed}
}

% geriSumRQ
\newcommand{\geriSumRQ}[2]{   
    \smallskip%
    \begin{mdframed}[hidealllines=true, backgroundcolor=gray!5]
        {\faSearch \hspace{0.2mm} \textbf{RQ\textsubscript{#1} Summary.} \textit{#2}}
    \end{mdframed}
}


% geriKeyPoint
\newcommand{\geriKeyPoint}[2]{   
    \smallskip%
    \begin{mdframed}[hidealllines=true, backgroundcolor=gray!5]
        {\faKey \hspace{0.2mm} \textbf{RQ\textsubscript{#1} Key Point.} \textit{#2}}
    \end{mdframed}
}

% Definizione macro: colora N righe
\newcount\rowcnt
\newcommand{\colorrows}[2]{%
  \rowcnt=0
  \loop
    \ifnum\rowcnt<#1
      \advance\rowcnt by 1
      \rowcolor{#2}%
      \ignorespaces
\relax
    \repeat
}

==> defs/title.tex <==
\title{A Systematic Literature Review on Smart Contract Vulnerabilities, Tools and Benchmarks}


==> figures/data/data.tex <==
\pgfplotstableread[col sep=comma,header=true]{% updated
Type,1,2,3,4,5
SLR,7,2,0,0,1
Survey,28,29,2,6,8
PS,93,81,9,8,3
}\tabA{}

\pgfplotstableread[col sep=comma,header=true]{% added header row
Type,1,2,3,4,5
0.2,8,37,3,13,12
0.4,0,13,0,0,0
0.5,20,7,7,0,0
0.8,35,8,0,0,0
1.0,65,47,1,1,0
}\tabB{}

\pgfplotstableread[col sep=comma,header=true]{% updated
Type,1,2,3,4,5
SLR,1,0,2,2,5
Survey,35,3,6,8,21
PS,37,10,26,33,88
}\tabC{}


\pgfplotstablecreatecol[
 create col/expr={
    \thisrow{1} + \thisrow{2} + \thisrow{3} +\thisrow{4}+\thisrow{5}
 }
]{sum}{\tabA}

\pgfplotstablecreatecol[
 create col/expr={
    \thisrow{1} + \thisrow{2} + \thisrow{3} +\thisrow{4}+\thisrow{5}
 }
]{sum}{\tabB}

\pgfplotstablecreatecol[
 create col/expr={
    \thisrow{1} + \thisrow{2} + \thisrow{3} +\thisrow{4}+\thisrow{5}
 }
]{sum}{\tabC}

==> figures/fig_criteria_pie.tex <==
\begin{figure*}[htbp]
\caption{Inclusion and Exclusion Criteria}
% \begin{tcolorbox}[colframe=black, colback=white, width=\textwidth, boxsep=2mm]
\centering
\label{fig:both_criteria}
\begin{minipage}[b]{0.5\textwidth}
  \centering
  \subcaption{Inclusion criteria}
  \label{fig:inclusion}
  \begin{tikzpicture}
    \pie[text=legend,pos={4,0},radius=1.7, sum=auto, rotate=0]{102/1-Criteria, 171/2-Criteria, 56/3-Criteria}
  \end{tikzpicture}
\end{minipage}%
\begin{minipage}[b]{0.5\textwidth}
  \centering
  \subcaption{Exclusion criteria}
  \label{fig:exclusion}
  \begin{tikzpicture}
    \pie[text=legend,pos={4,0},radius=1.7, sum=auto, rotate=0]{37/1-Criteria, 15/2-Criteria, 26/3-Criteria, 30/4-Criteria, 4/5-Criteria}
  \end{tikzpicture}
\end{minipage}
% \end{tcolorbox}
\end{figure*}


==> figures/fig_idqXclass_h.tex <==
\input{figures/data/data}
% Define styles for the plot
\pgfplotsset{
    a3 plot/.style={
    point meta=explicit,
    every node near coord/.append style={
      font=\footnotesize,
      color=black,
    },
    nodes near coords={
      \pgfmathtruncatemacro\iszero{\originalvalue==0}% <-- needed to remove space
      \ifnum\iszero=0
      \pgfmathprintnumber[fixed,fixed zerofill,precision=0]{\pgfplotspointmeta}
      \fi
    },
    xticklabel=\pgfmathprintnumber{\tick}\,$\%$,
    xmin=0,
    xmax=100.01, % added .01 
    visualization depends on={x \as \originalvalue},
    enlarge y limits={abs=6mm}
  },
    a3 series/.style={
    table/y expr=\coordindex, %added
    table/x expr=(\thisrow{#1}/\thisrow{sum}*100),
    table/meta=#1
    },
}

\begin{figure}[ht]
\caption{Distribution of IDQ scores per publication class}
\Description{Distribution of IDQ scores per publication class}
% \begin{tcolorbox}[colframe=black, colback=white, width=\linewidth, boxsep=2mm]
\centering
\footnotesize
\begin{tikzpicture}
\begin{axis}[
    xbar stacked, % Rotate bars horizontally
    height=4.1cm,
    width=7.3cm, % Adjust width for better visualization
    a3 plot, % Apply the defined style
    bar width=0.5cm,
    yticklabels from table={\tabC}{Type},
    ytick=data,
    xtick=\empty,
    y tick label style={
      rotate=0,
      anchor=east,
      yshift=0mm
    },
    legend style={
      at={(1.3,0.9)}, % Adjusted legend position for horizontal bars
      anchor=north,
      legend columns=1,
      draw=none,
      /tikz/every even column/.append style={text width=1cm, align=left},
    },
]
    \addplot [fill=palette1]    table[a3 series=1] {\tabC};
    \addplot [fill=palette2]    table[a3 series=2] {\tabC};
    \addplot [fill=palette3]    table[a3 series=3] {\tabC};
    \addplot [fill=palette4]    table[a3 series=4] {\tabC};
    \addplot [fill=palette5]    table[a3 series=5] {\tabC};

    % plot just to add total
    \addplot [forget plot,nodes near coords align=right] table[y expr=\coordindex,x expr=0.0001,meta=sum]{\tabC};

    \legend{\strut 0.2 , \strut 0.4, \strut 0.5, \strut 0.8, \strut 1.0}
\end{axis}

\end{tikzpicture}
% \end{tcolorbox}
\label{fig:distr_IDQ_class}
\end{figure}

==> figures/fig_idqXclass_v.tex <==
% A series
\pgfplotsset{
  a plot/.style={
    point meta=explicit,
    every node near coord/.append style={
      font=\tiny,
      color=black,
    },
    nodes near coords={
      \pgfmathtruncatemacro\iszero{\originalvalue==0}% <-- needed to remove space
      \ifnum\iszero=0
      \pgfmathprintnumber[fixed,fixed zerofill,precision=0]{\pgfplotspointmeta}
      \fi
    },
    yticklabel=\pgfmathprintnumber{\tick}\,$\%$,
    ymin=0,
    ymax=100.01, % added .01 
    visualization depends on={y \as \originalvalue},
    enlarge x limits={abs=6mm}
  },
    a series/.style={
    table/x expr=\coordindex, %added
    table/y expr=(\thisrow{#1}/\thisrow{sum}*100),
    table/meta=#1
    },
}


\begin{figure}
\caption{ Distribution of IDQ scores per publication class}
\label{fig:distr_IDQ_class}
\begin{tcolorbox}[colframe=black, colback=white, width=\linewidth, boxsep=2mm]
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar stacked,
    height=8cm,
    width=8cm,
    a plot,
    bar width=0.8cm, % increased from 0.3cm
    xticklabels from table={\tabC}{Type}, % read ticklabels from first column
    xtick=data,
    ytick=\empty,
    x tick label style={
      rotate=0,
      anchor=north, 
      xshift=-1mm, yshift=-1mm
    },
    legend style={
      at={(0.5,-0.25)},
      anchor=south,
      legend columns=-1,
      draw=none,
      /tikz/every even column/.append style={column sep=0.5cm}, % Spaziatura tra le colonne pari
      },]
    \addplot [fill=palette1, nodes near coords style={font=\large}]    table[a series=1] {\tabC};
    \addplot [fill=palette2, nodes near coords style={font=\large}]    table[a series=2] {\tabC};
    \addplot [fill=palette3, nodes near coords style={font=\large}]    table[a series=3] {\tabC};
    \addplot [fill=palette4, nodes near coords style={font=\large}]    table[a series=4] {\tabC};
    \addplot [fill=palette5, nodes near coords style={font=\large}]    table[a series=5] {\tabC};

    % plot just to add total
    \addplot [forget plot,nodes near coords align=above,nodes near coords style={font=\large}] table[x expr=\coordindex,y expr=0.0001,meta=sum]{\tabC};

    \legend{\strut 0.2 , \strut 0.4, \strut 0.5, \strut 0.8, \strut 1.0}
\end{axis}
\end{tikzpicture}
\end{tcolorbox}
\end{figure}

==> figures/fig_idqXvenue_h.tex <==
\input{figures/data/data}
% Define styles for the plot
\pgfplotsset{
    b2 plot/.style={
    point meta=explicit,
    every node near coord/.append style={
      font=\footnotesize,
      color=black,
    },
    nodes near coords={
      \pgfmathtruncatemacro\iszero{\originalvalue==0}% <-- needed to remove space
      \ifnum\iszero=0
      \pgfmathprintnumber[fixed,fixed zerofill,precision=0]{\pgfplotspointmeta}
      \fi
    },
    xticklabel=\pgfmathprintnumber{\tick}\,$\%$,
    xmin=0,
    xmax=110.01, % added .01 
    visualization depends on={x \as \originalvalue},
    enlarge y limits={abs=6mm}
  },
    b2 series/.style={
    table/y expr=\coordindex, %added
    table/x expr=(\thisrow{#1}*0.85),
    table/meta=#1
    },
}

\begin{figure}[ht]
\caption{Number of publications per IDQ score, by publication venue}
\Description{Number of publications per IDQ score, by publication venue}
\label{fig:distr_IDQ_venue}
% \begin{tcolorbox}[colframe=black, colback=white, width=\linewidth, boxsep=2mm]
\centering
\footnotesize
\begin{tikzpicture}
\begin{axis}[
    xbar stacked, % Rotate bars horizontally
    height=5cm,
    width=9.2cm, % Adjust width for better visualization
    bar width=0.4cm,
    yticklabels from table={\tabB}{Type},
    ytick=data,
    xtick=\empty,
    y tick label style={
      rotate=0,
      anchor=east,
      yshift=0mm
    },
    legend style={
      at={(0.5,-0.15)},
      anchor=north,
      legend columns=-1, 
      draw=none,
      align=center, % Centra il testo
      /tikz/every even column/.append style={align=left},
      },
    b2 plot, % Apply the defined style
]
    \addplot [fill=palette1]    table[b2 series=1] {\tabB};
    \addplot [fill=palette2]    table[b2 series=2] {\tabB};
    \addplot [fill=palette3]    table[b2 series=3] {\tabB};
    \addplot [fill=palette4]    table[b2 series=4] {\tabB};
    \addplot [fill=palette5]    table[b2 series=5] {\tabB};

    % plot just to add total
    \addplot [forget plot,nodes near coords align=right] table[y expr=\coordindex,x expr=0.0001,meta=sum]{\tabB};

    \legend{\strut Journal Article, \strut Proceeding, \strut Book Section, \strut Preprint, \strut Thesis/ Seminar Paper}
\end{axis}
\end{tikzpicture}
% \end{tcolorbox}
\end{figure}

==> figures/fig_quality_ps.tex <==
\begin{figure}[ht]
\centering
\footnotesize
\caption{Quality Appraisal of Primary Studies}
\label{fig:quality_ps}
% \begin{tcolorbox}[colframe=black, colback=white, width=\linewidth, boxsep=2mm]
\begin{tikzpicture}
\pie[text=legend,pos={4,0},radius=1.5, sum=auto, rotate=0]{39/Selected High, 55/Selected Medium,  0/Reclassified, 2/Duplicate, 85/Rejected}
\end{tikzpicture}
% \end{tcolorbox}
\end{figure}

==> figures/fig_quality_surveys.tex <==
\begin{figure}[h]
\centering
\footnotesize
\caption{Quality Appraisal of Surveys}
\label{fig:quality_surveys}
% \begin{tcolorbox}[colframe=black, colback=white, width=\linewidth, boxsep=2mm]
\begin{tikzpicture}
\pie[text=legend, pos={4,0}, sum=auto, radius=1.5]{10/Selected High, 6/Selected Medium, 4/Reclassified, 2/Duplicate, 57/Rejected}
\end{tikzpicture}
% \end{tcolorbox}
\end{figure}

==> figures/fig_venueXclass_h.tex <==
\input{figures/data/data}
\pgfplotsset{
  a2 plot/.style={
    point meta=explicit,
    every node near coord/.append style={
      font=\footnotesize,
      color=black,
    },
    nodes near coords={
      \pgfmathtruncatemacro\iszero{\originalvalue==0}% <-- needed to remove space
      \ifnum\iszero=0
      \pgfmathprintnumber[fixed,fixed zerofill,precision=0]{\pgfplotspointmeta}
      \fi
    },
    xticklabel=\pgfmathprintnumber{\tick}\,$\%$,
    xmin=0,
    xmax=100.01, % added .01 
    visualization depends on={x \as \originalvalue},
    enlarge y limits={abs=6mm}
  },
    a2 series/.style={
    table/y expr=\coordindex, %added
    table/x expr=(\thisrow{#1}/\thisrow{sum}*100),
    table/meta=#1
    },
}

\begin{figure}[ht]
\caption{Distribution of publication venues per publication class}
\Description{Distribution of publication venues per publication class}

% \begin{tcolorbox}[colframe=black, colback=white, width=\linewidth, boxsep=2mm]
\centering
\footnotesize
\begin{tikzpicture}
\begin{axis}[
    xbar stacked, % Change here
    height=3.9cm,
    width=9.2cm, % Adjusted width for better visualization
    bar width=0.4cm,
    yticklabels from table={\tabA}{Type}, % Changed to yticklabels
    ytick=data, % Changed to ytick
    xtick=\empty, % No x ticks
    y tick label style={
      rotate=0,
      anchor=east, % Adjusted anchor for horizontal bars
      yshift=0mm % Adjusted yshift for horizontal bars
    },
    legend style={
      at={(0.5,-0.15)},
      anchor=north,
      legend columns=-1, 
      draw=none,
      align=center, % Centra il testo
      /tikz/every even column/.append style={align=left},
      },
    a2 plot, % Apply the defined style
]
    \addplot [fill=palette1]  table[a2 series=1] {\tabA};
    \addplot [fill=palette2]  table[a2 series=2] {\tabA};
    \addplot [fill=palette3]  table[a2 series=3] {\tabA};
    \addplot [fill=palette4]  table[a2 series=4] {\tabA};
    \addplot [fill=palette5]  table[a2 series=5] {\tabA};
    % plot just to add total
    \addplot [forget plot,nodes near coords align=right] table[y expr=\coordindex,x expr=0.0001,meta=sum]{\tabA};

    \legend{\strut Journal Article, \strut Proceeding, \strut Book Section, \strut Preprint, \strut Thesis/ Seminar Paper}
    
\end{axis}
\end{tikzpicture}
% \end{tcolorbox}
\label{fig:distr_venue_class}
\end{figure}

==> tables/dataset.tex <==
{
\tiny
\rowcolors{2}{gray!5}{white}
\begin{longtable}{ccp{3.4cm}ccccccc} 
    \caption{
    A List of the Benchmarks Used in the Literature.
    } 
    \label{tab:benchmarks}\\
    \toprule
    \textbf{Discussed in} & \textbf{Publication} & \textbf{Tools} & \textbf{Link} & \textbf{\#Contracts} & \textbf{Results} & \textbf{Source Code} & \textbf{Bytecode} & \textbf{Addresses} \\ 
    \midrule
    \endfirsthead
    \midrule
    \multicolumn{10}{l}{{Continued from previous page}} \\
    \toprule
    \textbf{Discussed in} & \textbf{Publication} & \textbf{Tools} & \textbf{Link} & \textbf{\#Contracts} & \textbf{Results} & \textbf{Source Code} & \textbf{Bytecode} & \textbf{Addresses} \\ 
    \midrule
    \endhead
    \midrule
    \multicolumn{10}{r}{{Continued on next page}} \\
    \midrule
    \endfoot
    \bottomrule
    \endlastfoot
        \citeA{PiantadosiEtAl2022} & \cite{AshouriEtAl2020} &~&~& 12 &~&~& \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{AzzopardiEtAl2018} &~&~&~&~&~&~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{BhargavanEtAl2016} &~&~& 112,802 &~&~& \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{ChangEtAl2019} & sCompile &~& 36,099 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{ChapmanEtAl2019} & Deviant &~& 3 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{ChatterjeeEtAl2019} &~&~& 36,764 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{ChenEtAl2017} &~&~& 16,000 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{DongEtAl2019} &~&~& 2 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{El-DosukyEtAl2019} & DOORchain &~&~&~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{FeistEtAl2019} & Slither &~& 36,000 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{FuEtAl2019} &~&~& 10,000 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{GaoEtAl2019} & Easyflow &~&~&~&~& \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{GrechEtAl2018} & MadMax &~&~&~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{GrossmanEtAl2017} &~&~& 3,444,354 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{HeEtAl2019} &~&~& 18,498 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{HiraiEtAl2017} &~&~&~&~&~& \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{HonigEtAl2019} &~&~&~&~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{JiaoEtAl2020} &~&~& 482 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{LahbibEtAl2020} &~&~&~&~&~& \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{LaiEtAl2020} &~&~& 7,000 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{LiEtAl2019} & MuSC &~&~&~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{MaEtAl2019} & EVM* &~& 10 &~&~& \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{MedeirosEtAl2019} & SolUnit &~&~&~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{MomeniEtAl2019} &~&~& 13,745 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{MossbergEtAl2019} & Manticore &~& 100 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{NguyenEtAl2019} &~&~&~&~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{NikolicEtAl2018} &~&~& 970,898 &~&~& \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{ParkEtAl2018} &~&~&~&~&~& \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{PengEtAl2019} & SIF, SolAnalyser, Oyente, Securify, Maian, SmartCheck, Mythril &~& 1,838 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{SergeyEtAl2019} &~&~&~&~& \ding{51} & \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{ShishkinEtAl2018} &~&~&~&~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{TianEtAl2019} &~&~& 20 &~&~& \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{TorresEtAl2018} & Osiris & \href{https://github.com/christoftorres/Osiris/tree/master/datasets}{url} & 50,535 & \ding{51} &~& \ding{51} & \ding{51} \\ 
        \citeA{PiantadosiEtAl2022} & \cite{TsankovEtAl2018} & Solidify &~& 24,594 & \ding{51} &~& \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{TsankovEtAl2018} & Solidify &~& 100 & \ding{51} & \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{WangEtAl2020} &~&~&~&~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{YeEtAl2020} &~&~& 31,097 &~&~& \ding{51} &~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{ZhangQEtAl2020} &~&~& 49,522 &~& \ding{51} &~&~\\ 
        \citeA{PiantadosiEtAl2022} & \cite{ZhangYEtAl2020} &~&~& 2,214,409 &~&~& \ding{51} &~\\ 
        \citeA{dZaazaaAndElBakkali2023b, PiantadosiEtAl2022} & \cite{SongEtAl2019} & Oyente, ContractWard &~& 49,502 &~& \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b, PiantadosiEtAl2022} & \cite{GaoEtAl2021} & Deckard, SmartCheck, SMARTEMBED & \href{https://drive.google.com/file/d/13iTTpt7gFd9wEW35C2fX4pVT7cVlHgxi/view?usp=sharing}{url} & 22,725 &~& \ding{51} &~& \ding{51} \\ 
        \citeA{dZaazaaAndElBakkali2023b, PiantadosiEtAl2022} & \cite{TikhomirovEtAl2018} & Smartcheck & \href{https://github.com/smartdec/smartcheck/tree/master/src/test/resources/rules}{url} & 4,600 &~& \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b, PiantadosiEtAl2022} & \cite{WangEtAl2019} & NPChecker, Securify, Oyente, Mythril &~& 30,000 &~& \ding{51} & \ding{51} &~\\ 
        \citeA{dZaazaaAndElBakkali2023b} &~& Smartcheck, Oyente, Mythril, Securify, Slither, Osiris, DeeSCVHunter & \href{https://github.com/Messi-Q/Smart-Contract-Dataset}{url} &~&~& \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} &~& Smartcheck, Oyente, Mythril, Securify, Slither, Osiris, DeeSCVHunter & \href{ https://drive.google.com/file/d/1XFp3tZSMkWSkeLSHe\_vrQjGZYZ3LzB2s/view}{url} &~&~& \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} &~& Smartcheck, Oyente, Mythril, Securify, Slither, Osiris, DeeSCVHunter & \href{https://drive.google.com/file/d/1UhHHevE9iDmvSB\_k\_lhyI58KAj7hnB1o/view}{url} &~&~& \ding{51} & \ding{51} &~\\ 
        \citeA{dZaazaaAndElBakkali2023b} &~& Slither & \href{https://www.kaggle.com/datasets/bigquery/ethereum-blockchain/}{url} &~&~&~&~& \ding{51} \\ 
        \citeA{dZaazaaAndElBakkali2023b} &~& Yingjie et al., SmartBugs, SolidiFI & \href{https://github.com/DependableSystemsLab/SolidiFI-benchmark/tree/master/buggy\_contracts}{url} &~& \ding{51} & \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{QianEtAl2020} & VulDeeSmartContract (BLSTM-ATT), Securify, SmartCheck, Mythril, Oyente & \href{https://github.com/Messi-Q/ReChecker, https://drive.google.com/file/d/1h9aFFSsL7mK4NmVJd4So7IJlFj9u0HRv/view}{url} &~& \ding{51} & \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{LiaoEtAl2019} & SoliAudit, Oyente, Remix & \href{https://goo.gl/UAUpK5/}{url} & 21,044 &~&~&~& \ding{51} \\ 
        \citeA{dZaazaaAndElBakkali2023b} & \citeA{WuHEtAl2021} & Peculiar & \href{https://github.com/wuhongjun15/Peculiar/blob/main/dataset.zip}{url} & 40,742 & \ding{51} & \ding{51} &~& \ding{51} \\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{AshrafEtAl2020} & GasFuzzer & \href{https://github.com/TechBeatle/EthereumSmartContractsDataset}{url} & 3,170 &~&~&~& \ding{51} \\ 
        \citeA{dZaazaaAndElBakkali2023b} & \citeA{SamreenAndAlalfi2021} & SmartScan, SmartCheck &~& 500 &~&~&~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \citeA{NguyenEtAl2021} & SGUARD &~& 5,000 &~&~&~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \citeA{PanEtAl2021} & ReDefender &~& 204 &~&~&~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \citeA{PanEtAl2021} & ReDefender &~& 395 &~&~&~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \citeA{ControEtAl2021} & EtherSolve &~& 1,000 &~&~&~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \citeA{AshizawaEtAl2021} & Eth2Vec &~& 95,152 &~&~&~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \citeA{ZhouEtAl2021} & SMARTGIFT &~&~&~&~&~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \citeA{LiuZEtAl2021} & AME (CGE) &~& 40,932 &~& \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{JianjunEtAl2021} & Jianjun et al tool &~& 2,000,000 &~&~& \ding{51} &~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{FerreiraEtAl2020} & ÆGIS, ECFChecker, Sereum &~& 675,444 &~& \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{Hwang2020} & SC Analyzer & \href{https://github.com/sjmini/icse2020-Solidity}{url} & 55,046 &~& \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{NguyenEtAl2020} & sfuzz, ContractFuzzer, Oyente &~& 4,112 &~& \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{WangEtAl2020Artemis} & Artemis, Maian &~& 12,899 &~& \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{HaoEtAl2020} & SCScan &~& 1,000 &~& \ding{51} &~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{XueEtAl2021} & Clairvoyance, Slither, Oyente, Securify & \href{Clairvoyance — Clairvoyance documentation (toolman-demo.readthedocs.io)}{url} & 11,714 & \ding{51} & \ding{51} &~& \ding{51} \\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{FerreiraEtAl2021} & Smartbugs & \href{https://github.com/smartbugs/smartbugs-wild}{url} & 47,398 & \ding{51} & \ding{51} &~& \ding{51} \\ 
        \citeA{diAngeloAndSalzer2023} & \cite{FerreiraEtAl2021} & SmartBugs & \href{https://github.com/smartbugs/smartbugs-curated}{url} & 143 &~& \ding{51} &~&~\\
        \citeA{dZaazaaAndElBakkali2023b} & \cite{AlbertEtAl2019} & SAFEVM, VeryMax, SeaHorn, CPAchecker, Oyente, EthIR & \href{https://github.com/costa-group/EthIR/tree/master/examples/safevm/all}{url} & 24,294 &~& \ding{51} &~& \ding{51} \\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{AlbertEtAl2019} & SAFEVM & \href{https://github.com/costa-group/EthIR/tree/master/examples/safevm/subset0x00-0x01/original}{url} & 29 &~& \ding{51} &~& \ding{51} \\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{ChenEtAl2019} & OYENTE, MAIAN, Mythril, Evmdis, Miasm, Porosity &~& 4,979,625 &~&~&~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{PrechtelEtAl2019} & Mythril-enhanced version &~& 167,698 & \ding{51} &~&~&~\\ 
        \citeA{dZaazaaAndElBakkali2023b} & \cite{EnceEtAl2018} & SASC, oyente &~& 2,952 &~&~&~&~\\ 
        \citeA{diAngeloAndSalzer2023} & \cite{SchneidewindEtAl2020} & eThor & \href{https://owncloud.tuwien.ac.at/index.php/s/qNq87OBHnyOuru2/download}{url} & 720 &~&~& \ding{51} & \ding{51} \\ 
        \citeA{diAngeloAndSalzer2023} & \cite{ZhouEtAl2020} & EverEvolvingG & \href{https://drive.google.com/file/d/1xLssDxYWyKFCwS5HUrQaSex0uwJRSvDi/view}{url} & 344 &~& \ding{51} &~& \ding{51} \\ 
         
       ~& \citeA{diAngeloAndSalzer2023} &~& \href{https://github.com/gsalzer/cgt}{url} & 4,859 &~& \ding{51} & \ding{51} & \ding{51} \\ 
       ~& \citeA{JeonEtAl2023} & SmartConDetect & \href{https://github.com/s00ne/SmartConDetect?tab=readme-ov-file}{url} & 10,000 &~& \ding{51} &~&~\\ 
       ~& \citeA{ChaliasosEtAl2024} &~& \href{https://github.com/StefanosChaliasos/sc-defi-security/tree/main/dataset}{url} &~& \ding{51} & \ding{51} & \ding{51} & \ding{51} \\ 
       ~& \citeA{LiEtAl2022} & SmartFast & \href{https://github.com/SmartContractTools/SmartFast/tree/main/Dataset1}{url} & 149 & \ding{51} & \ding{51} &~&~\\ 
       ~& \citeA{LiEtAl2022} & SmartFast & \href{https://github.com/SmartContractTools/SmartFast/tree/main/Dataset2}{url} & 13,509 & \ding{51} & \ding{51} &~& \ding{51} \\ 
       ~& \citeA{NguyenEtAl2023} & MANDO-HGT, MANDO-GURU & \href{https://github.com/MANDO-Project/ge-sc-transformer/tree/main/data}{url} &~& \ding{51} & \ding{51} &~&~\\ 
       ~& \citeA{NguyenEtAl2023} & MANDO-HGT, MANDO-GURU & \href{https://github.com/MANDO-Project/ge-sc-transformer/tree/main/experiments/ge-sc-data/}{url} &~& \ding{51} & \ding{51} & \ding{51} & \ding{51} \\ 
       ~& \citeA{JiamingYeEtAl2022} & Vulpedia & \href{https://drive.google.com/file/d/1kizsz0\_8B8nP4UNVr0gYjaj25VVZMO8C/edit}{url} &~&~&~&~&~\\ 
       ~& \citeA{GuoEtAl2024} & MEVD & \href{https://github.com/COPELONG/MEVD}{url} &~& \ding{51} & \ding{51} &~&~\\ 
       ~& \citeA{DuanEtAl2023} & Duan et al. Framework & \href{https://github.com/Sheep-L/boke}{url} &~&~&~&~&~\\ 
       ~& \citeA{QianEtAl2023b} & RNVulDet & \href{https://github.com/Messi-Q/RNVulDet/tree/main/dataset}{url} &~&~&~&~& \ding{51} \\ 
       ~& \citeA{SoudEtAl2023} & SmartState & \href{https://github.com/InPlusLab/SmartState-dataset}{url} &~&~& \ding{51} &~& \ding{51} \\ 
       ~& \citeA{ChoiEtAl2021} & Smartian & \href{https://github.com/SoftSec-KAIST/Smartian-Artifact/tree/main/benchmarks}{url} &~&~& \ding{51} & \ding{51} & \ding{51} \\ 
       ~& \citeA{HajiHosseinKhaniEtAl2024} & SCsVulLyzer &~&~&~& \ding{51} &~&~\\ 
       ~& \citeA{L.ZhangEtAl2022} & MODNN & \href{https://github.com/yangzuwjl/MODNN}{url} & 18,796 &~& \ding{51} &~&~\\ 
       ~& \citeA{DaiEtAl2022} & SuperDetector & \href{https://github.com/xf97/HuangGai/tree/master/injectedContractDataSet}{url} &~&~& \ding{51} &~& \ding{51} \\ 
       ~& \citeA{DaiEtAl2022} & SuperDetector & \href{https://github.com/xf97/HuangGai/tree/master/manualCheckDataset}{url} &~&~& \ding{51} &~& \ding{51} \\ 
       ~& \citeA{HuEtAl2023b} & SoliDetector & \href{https://github.com/1052445594/SoliDetector}{url} &~&~& \ding{51} &~& \ding{51} \\ 
       ~& \citeA{NassirzadehEtAl2021} & Gas Gauge & \href{https://github.com/gasgauge/gasgauge.github.io/tree/main/Benchmark}{url} &~& \ding{51} & \ding{51} &~& \ding{51} \\ 
       ~& \citeA{sigmaprime_solidity_security} &~& \href{https://blog.sigmaprime.io/solidity-security.html\#unchecked-calls-vuln}{url} &~&~& \ding{51} &~&~\\ 
       ~& \citeA{QianEtAl2023c} &~& \href{https://github.com/Messi-Q/Cross-Modality-Bug-Detection/tree/main/bytecode}{url} &~&~&~& \ding{51} &~\\ 
       ~& \citeA{QianEtAl2023c} &~& \href{https://github.com/Messi-Q/Cross-Modality-Bug-Detection/tree/main/sourcecode}{url} &~&~& \ding{51} &~&~\\ 
       ~& \citeA{SunEtAl2022b} & ConFuzzius-BI & \href{https://github.com/SmartcontractTest/ConFuzzius-BI/tree/main/dataset/asset-related/realworld}{url} & 43 &~& \ding{51} &~&~\\ 
       ~& \citeA{SunEtAl2022b} & ConFuzzius-BI & \href{https://github.com/SmartcontractTest/ConFuzzius-BI/tree/main/dataset/asset-related/manuinject/All}{url} & 19 &~& \ding{51} &~& \ding{51} \\ 
       ~& \citeA{WeiEtAl2023} &~& \href{https://github.com/WeiZ-boot/Smartcontract-benchmark}{url} & 110 & \ding{51} & \ding{51} &~&~\\ 
       ~& \citeA{diAngeloEtAl2024} &~& \href{https://github.com/gsalzer/skelcodes/tree/main}{url} & 248,328 &~& \ding{51} & \ding{51} & \ding{51} \\ 

       ~& \citeA{sun2024gptscan} & Top200 & \href{https://github.com/MetaTrustLabs/GPTScan-Top200}{url} &~&~&~&~&~\\
       ~& \citeA{sun2024gptscan} & Web3Bugs & \href{https://github.com/ZhangZhuoSJTU/Web3Bugs}{url} &~&~&~&~&~\\
       ~& \citeA{sun2024gptscan} & DefiHacks & \href{https://wooded-meter-1d8.notion.site/0e85e02c5ed34df3855ea9f3ca40f53b?v=22e5e2c506ef4caeb40b4f78e23517ee}{url} & 101 & \ding{51} & \ding{51} &~& \ding{51} \\
       ~& \citeA{luo2024scvhunter} & SCVHunter & \href{https://figshare.com/articles/software/scvhunter/24566893/1?file=43154218}{url} & 1,200 & \ding{51} & \ding{51} &~& \ding{51} \\
       ~& \citeA{li2024cobra} & Cobra & \href{https://figshare.com/articles/dataset/dataset/22313074 }{url} &~&~&~&~&~\\
       ~& \citeA{wu2024advscanner} & AdvSCanner & \href{https://figshare.com/s/3f864a6e7c6245ad9704}{url} &~& \ding{51} & \ding{51} &~&~\\
       ~& \citeA{wang2024contracttinker} & ContractTinker & \href{https://github.com/CheWang09/LLM4SMAPR/tree/main/open_source_dataset }{url} &~&~&~&~&~\\
       ~& \citeA{eshghie2024oracle} & XploGen & \href{https://github.com/mojtaba-eshghie/XploGen/tree/main/benchmarks/supported_tools/ExGen/benchmark }{url} &~& \ding{51} & \ding{51} &~&~\\
       ~& \citeA{liu2024funredisp, liu2024funredisp2} & FunRedisp & \href{https://zenodo.org/records/12671411 }{url} &~&~&~& \ding{51} &~\\
       ~& \citeA{chen2024identifying} & SOChecher & \href{https://github.com/BugmakerCC/SOChecker }{url} &~&~&~&~&~\\
       ~& \citeA{liang2024towards} & PonziGuard & \href{https://github.com/PonziDetection/SmartPonzi/tree/main/dataset}{url} &~& \ding{51} & \ding{51} &~&~\\
       ~& \citeA{guo2024smart} & RLRep & \href{https://github.com/Anonymous123xx/RLRep}{url} &~& \ding{51} & \ding{51} &~&~\\
       ~& \citeA{liu2024automated} & InvCon+ & \href{https://github.com/Franklinliu/InvConPlus-Tool/tree/main}{url} &~& \ding{51} & \ding{51} &~&~\\
        \citeA{wu2024we} & \citeA{ren2021empirical} &~& \href{https://github.com/renardbebe/Smart-Contract-Benchmark-Suites}{url} & 46,186 &~& \ding{51} &~&~\\
       ~& \citeA{TorresEtAl2021} & ConFuzzius & \href{https://github.com/christoftorres/ConFuzzius/tree/master/dataset/etherscan}{url} & 21,000 &~& \ding{51} &~&~\\
       ~& \citeA{TorresEtAl2021} & ConFuzzius & \href{https://github.com/christoftorres/ConFuzzius/tree/master/dataset/curated}{url} & 128 &~& \ding{51} &~&~\\
       ~& \citeA{Zheng2023rudder} & SliSE & \href{https://github.com/InPlusLab/ReentrancyStudy-Data}{url} & 34 & \ding{51} & \ding{51} &~& \ding{51} \\
       ~& \citeA{Z.ZhangEtAl2023} & Code4rena & \href{https://code4rena.com/}{url} &~&~&~&~&~\\
       ~& \citeA{liao2024smartaxe} & SmartAxe & \href{https://github.com/InPlusLab/FSE24-SmartAxe}{url} &~&~& \ding{51} & \ding{51} &~\\
       ~& \citeA{hajihosseinkhani2024unveiling} & BCCC-SCsVul-2024 & \href{https://www.yorku.ca/research/bccc/ucs-technical/cybersecurity-datasets-cds/}{url} &~&~& \ding{51} &~&~\\
       ~& \citeA{qian2024mufuzz} & MuFuzz & \href{https://drive.google.com/file/d/1h_XYXcKqfKuN7ArsXDwFq52V_mH3GQ5w/view }{url} &~&~& \ding{51} &~&~\\
       ~& \citeA{wang2024contractgnn} & ContractGNN & \href{https://github.com/Wang-Yi-chen/ContractGNN }{url} &~&~&~&~&~\\
       ~& \citeA{chu2024deepfusion} & DeepFusion & \href{https://github.com/Tourneso/DeepFusion }{url} &~&~&~&~&~\\
       ~& \citeA{li2024static} &~& \href{https://sites.google.com/view/sc-sast-study-fse2024/benchmark-construction }{url} & 788 &~& \ding{51} &~&~\\
       ~& \citeA{zheng2024dappscan} & DAppSCAN-source & \href{https://github.com/InPlusLab/DAppSCAN/tree/main/DAppSCAN-source}{url} & 21,457 & \ding{51} & \ding{51} &~&~\\
       ~& \citeA{zheng2024dappscan} & DAppSCAN-bytecode & \href{https://github.com/InPlusLab/DAppSCAN/tree/main/DAppSCAN-bytecode}{url} & 21,457 & \ding{51} &~& \ding{51} &~\\
\end{longtable}
}

==> tables/full_taxonomy.tex <==
\scriptsize
\onecolumn
\begin{longtable}{p{0.3cm} p{2.9cm} p{8.3cm} p{5.1cm}}
    \caption{A comprehensive list of vulnerabilities hierarchical organized.}
    \label{tab:full_tax}\\
    \toprule
    \textbf{Id} & \textbf{Name} & \textbf{Description} & \textbf{Alternative names} \\ 
    \midrule
    \endfirsthead
    \multicolumn{4}{c}{{Continued from previous page}} \\
    \toprule
    \textbf{Id} & \textbf{Name} & \textbf{Description} & \textbf{Alternative names} \\ 
    \midrule
    \endhead
    \midrule
    \multicolumn{4}{r}{{Continued on next page}} \\
    \midrule
    \endfoot
    \bottomrule
    \endlastfoot

    \multicolumn{4}{l}{\textbf{1 - Malicious Environment, Transactions or Input}}\\
    \midrule
    
        1A
        & Call to the unknown \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, KushwahaEtAl2022a}
        & An unrestricted CALL to an unknown address may lead to the execution of malicious code, e.g. the fallback function of the called contract. This vulnerability is a generalization of 1A Reentrancy, where the callee executes a call back to the caller.
        & Unexpected fallback function \cite{Rameder2022} \\

        1A1
        & Reentrancy \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, ChoiEtAl2021, ChuEtAl2023, ZhouEtAl2022, KushwahaEtAl2022b, Staderini2022, ChaliasosEtAl2024}
        & The callee calls back the caller before the initial call completes and necessary checks and state changes occur. A typical example is an Ether transfer to a contract with a fallback function crafted to reenter the original function.
        & Reentrancy-eth \citeA{AgarwalEtAl2022}\cite{slither}, Cross function race condition, Recursive call vulnerability, Race to empty \cite{Rameder2022}\\
        
        1B 
        & Exact balance dependency \cite{Rameder2022}
        & If a contract relies on maintaining an exact balance in storage rather than querying the environment, attackers can manipulate it by increasing its balance without executing its code.
        & Unexpected Ether, Manipulated balance,
        Unexpected Balance \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Unexpected Ether balance \citeA{MunirAndTaha2023},
        Unprotected Ether Balance \citeA{Staderini2022}, 
        Balance equality \citeA{AgarwalEtAl2022},
        Strict Balance Equality \citeA{ChenEtAl2022}\\

        1B1
        & Forcing Ether to contracts \cite{Rameder2022}
        & Attackers can manipulate a contract's balance without executing its code by designating the contract's address as the beneficiary of a SELFDESTRUCT operation or as the recipient of a mining reward. 
        & Check on force to receive balance \citeA{DiasEtAl2021} \\

        1B2
        & Pre-sent Ether \cite{Rameder2022}
        & Attackers can manipulate a contract's balance without executing its code by predicting its address and sending Ether before the contract is deployed. Toward the sender's address and the nonce of the transaction that creates the contract is possible to predict a contract's address. 
        & \\
        
        1C 
        & Improper data validation \cite{Rameder2022} 
        & Failing to validate data from untrusted sources, such as external libraries or contracts, before use.
        & Untrustworthy data feeds \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, KushwahaEtAl2022a}\\

        1D 
        & Vulnerable Delegatecall \cite{Rameder2022} 
        & Performing a DELEGATECALL or CALLCODE to an untrusted address executes code in the caller’s context. A malicious callee can alter the caller’s state variables and gain complete control over its balance.
        & Delegate call to Untrusted Callee \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023}, Delegate call to Insecure Contracts \citeA{ZhouEtAl2022}, Unsafe delegatecall \citeA{WeiEtAl2023}, check on target address in delegatecall \citeA{DiasEtAl2021}, Delegate call \citeA{AgarwalEtAl2022, KushwahaEtAl2022a, KushwahaEtAl2022b} \\

        \midrule
        \multicolumn{4}{l}{\textbf{2 - Blockchain/Environment Dependency}}\\
        \midrule

        2A
        & Block State Dependency \citeA{ChenEtAl2022, ChoiEtAl2021}
        & Contract logic should avoid using block information for precise calculations or critical time dependencies. Miners can influence these values, which may also be affected by network conditions or intentional manipulation, leading to inconsistencies and vulnerabilities in contract behavior.
        & Block Info Dependency \citeA{ChenEtAl2022}\\

        2A1
        & Timestamp dependency \cite{Rameder2022} \citeA{ ChuEtAl2023, ZhouEtAl2022, KushwahaEtAl2022a, KushwahaEtAl2022b, Staderini2022}
        & The block's timestamp should not be used for precise calculations or critical time dependencies in the contract logic. Miners have control over this value and can manipulate it to a certain extent, or the value may be subject to changes for other reasons. In the context of Ethereum Blockchain, nodes are allowed to submit a value up to 900ms error.
        & Time constraints, Time manipulation \cite{Rameder2022}, Time restriction\citeA{VivarEtAl2021}, Block values as a proxy for time\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} \\

        2A2
        & Block number dependency \cite{Rameder2022}
        & Using the block number bears similar risks as using other block information like the timestamp and should not be used in critical operations, as miners can also manipulate the block number. 
        & \\

        2A3
        & Blockhash dependency \cite{Rameder2022}
        & Blockhash usage vulnerability results from the usage, in critical operations, of blockhash variables. A malicious miner can manipulate this value.
        & Blockhash usage\citeA{Staderini2022} \\

        2B 
        & Transaction-ordering dependency \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, AgarwalEtAl2022, ZhouEtAl2022, ChuEtAl2023, KushwahaEtAl2022a, KushwahaEtAl2022b}
        & Contract logic should not depend on the order of transactions within a block, as miners can arrange them in any sequence, potentially for malicious purposes. Additionally, the contract's state can change between transaction submission and block inclusion, as miners may prioritize other transactions, even if they were submitted later.
        & Event-ordering bugs \cite{Rameder2022}\\

        2B1
        & Front-running attack \cite{Rameder2022}
        & Transactions are prioritized by miners based on their gas prices. For example, in a contract that rewards a player for guessing an answer, an attacker can monitor the mempool for such transactions. By submitting a higher gas price transaction with the same solution, the attacker can front-run the original transaction, ensuring the transaction is processed first.
        & Race condition \cite{Rameder2022}\\
        
        2C 
        & Bad random number generation \cite{Rameder2022}
        & Random numbers are crucial for applications like lotteries and games but are challenging to generate securely. Relying on global blockchain variables, such as timestamps, as seeds is risky because miners can manipulate these values. Additionally, other transactions within the same block or contracts called in the same transaction can access these global variables and potentially predict the random number.
        & Generating Randomness \cite{Rameder2022} \citeA{ ZhouEtAl2022, Staderini2022},
        Bad randomness \cite{Rameder2022},
        Weak Sources of Randomness from Chain Attributes \citeA{dZaazaaAndElBakkali2023a,dZaazaaAndElBakkali2023b}, Random Number\citeA{VivarEtAl2021}\\

        2C1
        & Randomness Using Block Hash \citeA{KushwahaEtAl2022a}
        & Randomness in blockchain operations can use block hashes, but this method is vulnerable to manipulation. Miners can influence block hashes by altering timestamps or other parameters, making the randomness predictable and potentially compromising security.
        & \\
        
        2D 
        & Leakage of confidential information \cite{Rameder2022} 
        & All transactions and contract states are visible to miners and anyone observing the blockchain, even if the visibility of variables is set to private or internal in the source code. Therefore, encryption and commitment schemes are important to protect secret information.
        & Lack of transaction privacy \cite{Rameder2022} \citeA{ KushwahaEtAl2022a},
        Private information leakage, Nothing is secret, Confidentiality failure, Keeping secrets, Data exposure \cite{Rameder2022},
        On-chain oracle manipulation \citeA{ChaliasosEtAl2024}, Secrecy failure \citeA{Staderini2022}, Exposed secret \citeA{MunirAndTaha2023}, Unencrypted private data on-chain \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}, Secrets\citeA{VivarEtAl2021} \\
    
        2E
        & Unpredictable state \cite{Rameder2022} \citeA{ VivarEtAl2021}
        & Calling contracts or libraries in a contract's business logic can lead to unpredictable effects. They can self-destruct, be updated later, and contain known vulnerabilities or, more simply, be an error when referring to them. The results are unpredictable effects. 
        & \\

        2E1
        & Dynamic Library \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & A smart contract relying on updatable components, such as other smart contracts or external libraries, may be vulnerable. If an attacker gains control over these components, they can alter the contract logic and exploit the system.
        & \\

        2E2
        & References to destroyed contracts \citeA{MunirAndTaha2023}
        & The address of a destroyed contract remains on the blockchain but no longer has any associated code or state. While you can still reference or use the address, it has limited functionality, and you cannot execute code or access any data associated with it.
        & \\

        2E3
        & Using components with known vulnerabilities\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Using existing libraries and open-source codes in a newly created project is a very useful practice to avoid reinventing the wheel. However, not all open-source codes and libraries are safe and they might contain vulnerabilities that could be exploited. Therefore, even if the newly created smart contract is secure, integrating these external codes may introduce hidden vulnerabilities.
        & \\

        2E4
        & External Contract Referencing \citeA{ZhouEtAl2022}
        & Solidity allows using any address for contracts, enabling malicious contracts to hide by providing incorrect addresses in constructors. For example, initializing an external library with a provided address during deployment may pass audits but poses security risks if the wrong address is used, potentially invoking malicious contracts. 
        & Misuse of address parameters in the constructor \citeA{MunirAndTaha2023}, Value assigned to contract address \citeA{DiasEtAl2021}\\

        \midrule
        \multicolumn{4}{l}{\textbf{3 - Exception \& Error Handling Disorders}}\\
        \midrule
        
        3A
        & Unchecked low-level call/send return values \cite{Rameder2022}
        & Low-level calls in Solidity do not raise an exception on failure but return a Boolean status. Failing to check this return status and handle errors appropriately can lead to critical vulnerabilities.
        & Unchecked call return values \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022, Staderini2022},
        Unchecked external calls \citeA{ChenEtAl2022},
        Check on external call \citeA{MunirAndTaha2023},
        Unchecked call \citeA{KushwahaEtAl2022b},
        Unchecked send \cite{Rameder2022} \citeA{ Staderini2022, WeiEtAl2023},
        Unhandled exception \cite{Rameder2022} \citeA{ ChuEtAl2023},
        Improper handling of exceptions \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Unchecked/unsafe send \cite{Rameder2022}\\

        3A1
        & Send instead of transfer \cite{Rameder2022} \citeA{ MunirAndTaha2023}
        & The choice of ether transfer function affects both the transfer of gas and the execution of the caller (sender) contract because call.value(x) and send(x) do not throw an exception in case of a failed transfer. In contrast, transfer(x) throws an exception if the transaction is unsuccessful. This makes the use of send instead of transfer a vulnerability.
        & \\
        
        3B
        & Unexpected throw or revert \cite{Rameder2022}
        & Calls to other contracts may fail, throw exceptions, or revert the transaction. Failing to handle these situations adequately can lead to critical issues such as Denial of Service (DoS) or lost funds.
        & Unexpected-throw-DoS, DoS with unexpected revert/throw\cite{Rameder2022}, DoS with failed call \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023, KushwahaEtAl2022a}, Dos by External contracts \cite{Rameder2022} \citeA{ Staderini2022} \\

        3B1
        & Mishandled out-of-gas exception \cite{Rameder2022}
        & Calling another contract with too little gas will cause an out-of-gas exception, potentially resulting in a vulnerability if not handled properly. A typical example is using Solidity’s send method to transfer funds: the 2300 gas supplied with the call will lead to an out-of-gas exception if the recipient contract executes more than a few simple instructions. 
        & Gasless send\cite{Rameder2022} \citeA{ Staderini2022, KushwahaEtAl2022a}\\

        3C
        & Assert, require or revert violation \cite{Rameder2022}
        & Solidity’s error handling mechanisms—assert, require, and revert (or their bytecode counterparts)—must be used correctly to prevent abnormal function behavior. Proper use of these functions ensures that contracts fail safely and predictably, protecting against vulnerabilities and maintaining the integrity of the contract's state.
        & Assert violation \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Assertion failure \citeA{ChoiEtAl2021},
        Requirement violation \citeA{ChoiEtAl2021, WeiEtAl2023, Staderini2022},
        Requirement violation by the called smart contract \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Require on input variable \citeA{DiasEtAl2021},
        Revert require, Exception state \citeA{AgarwalEtAl2022}\\

        \midrule
        \multicolumn{4}{l}{\textbf{4 - Denial of Service}}\\
        \midrule

        4A
        & Greedy contract \cite{Rameder2022}
        & A smart contract can access assets through an external library, which may accidentally or maliciously self-destruct or lack the implementation of withdrawal functions, providing only deposit functions. This can result in the contract being unable to retrieve the assets, leading to potential loss or inaccessibility of funds.
        & Locked Ether \cite{Rameder2022},
        Freezing Ether \citeA{Staderini2022, ZhouEtAl2022, ChoiEtAl2021, KushwahaEtAl2022b}\\

        4A1
        & Locked Money \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022, ChuEtAl2023}
        & Smart contracts that implement payable functions but no withdrawal ones are vulnerable because they can lock money without the ability to get it back.  
        & \\

        4A2
        & Frozen Ether \cite{Rameder2022}
        & If a contract uses library code to access its assets, then accidental or malicious self-destruction of the library contract may render the assets inaccessible.
        & \\

        4B
        & Ether lost in transfer\cite{Rameder2022}
        & Ether sent to an unused address becomes inaccessible because there is no corresponding private key to manage or access it. Once sent, the funds cannot be retrieved or utilized. 
        & Transfer to orphan address \cite{Rameder2022},
        Lost of Ether \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, KushwahaEtAl2022a}, Loss of Ether \citeA{VivarEtAl2021}\\

        4C
        & DoS with block gas limit reached \cite{Rameder2022} \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, KushwahaEtAl2022a}
        & The total gas consumed by all transactions in a block is limited by the block gas limit. Transactions that exceed this limit will not be included or processed in that block.
        & DoS Costly Pattern and Loops \citeA{Staderini2022},
        Check on gas Limit \citeA{DiasEtAl2021},
        Gas limit in loops, Extra Gas in loop \citeA{AgarwalEtAl2022} \\

        4C1
        & Multiple calls in a single transaction \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Performing calls inside a loop, for example, could create a DOS. If one call throws, the whole execution stops. So if there is a loop on the user address, and one of them is a contract that implements a fallback function that simply reverts, a DOS attack will occur. \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Nested Call \citeA{ChenEtAl2022}, Multiple calls, Transfer in loop\citeA{AgarwalEtAl2022}\\
        
        4C2
        & Array length manipulation \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022}
        & In older versions of Solidity, it is possible to manipulate the length field of an array using standard arithmetic operations. For example, decrementing the length field with code like anArray.length-- can cause an underflow, setting the array length to the maximum integer value. This vulnerability can disable a contract.
        & \\
        
        4C3
        & Infinite loop \citeA{WeiEtAl2023}
        & In a loop's termination condition, unchecked user input or comparisons between integers of different sizes can cause the loop to exceed the block gas limit or become prohibitively expensive to complete. This can lead to transaction failures due to non-terminating loops or unbounded mass operations. 
        & Unbounded mass operation \citeA{MunirAndTaha2023} \\
        
        4D
        & DoS by Exception inside loop \cite{Rameder2022}
        & Operations inside loops that may throw exceptions and depend on external transactions to succeed are open to DoS attacks by malicious users.
        & DoS under external influence \cite{Rameder2022} \citeA{ ChenEtAl2022}, Wallet griefing causing out of gas exception \cite{Rameder2022} \\

        4E
        & Insufficient gas griefing \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023, WeiEtAl2023, KushwahaEtAl2022a}
        & A contract that relays input from the caller to another contract can be exploited if the caller provides just enough gas for the initial transaction but insufficient gas for the sub-call. This can lead to failures or unexpected behavior in the sub-call.
        & \\

        4F
        & Overpowered Role \citeA{AgarwalEtAl2022}
        & An "overpowered role" refers to a role with excessive control, such as an administrator with broad privileges. This centralization poses risks of abuse and security vulnerabilities. Developers should prevent any single role from having too much power.
        & Check on overpowered role \citeA{DiasEtAl2021} \\

        4G
        & Missed to implement a fallback function \citeA{MunirAndTaha2023}
        & The call.value(x) can be problematic if the recipient function is not explicitly specified. By default, call invokes the target contract's fallback function. If a malicious contract deliberately omits a fallback function, any deposits made to it will fail, causing DoS issues in the sender contract. 
        & \\
        
        \midrule
        \multicolumn{4}{l}{\textbf{5 - Resurce Consuption \& Gas Related Issues}}\\
        \midrule

        5A 
        & Gas costly loops \cite{Rameder2022}
        & Unbounded and costly operations in loops should be avoided to avoid inefficiency and potential DoS. 
        & Invariants in loops \cite{Rameder2022} \\

        5B
        & Gas costly pattern \cite{Rameder2022}
        & Smart contract code should avoid inefficient operations and gas-costly patterns to minimize gas consumption and reduce transaction costs.
        & \\

        5C
        & High gas consumption of variable data type or declaration
        & In Solidity, certain data types consume more gas than others, and a variable's visibility also influences gas consumption. These characteristics can contribute to excessive gas costs.
        & \\

        5C1
        & Byte Array \cite{Rameder2022}
        & In Solidity, the data type byte[] consumes more gas than a byte array due to padding rules.
        & Variable type \citeA{DiasEtAl2021}\\

        5C2
        & Invariant State variables not declared constant \cite{Rameder2022} 
        & Invariants not declared constant consume more gas than necessary.
        & Declaration of invariant state variable \citeA{DiasEtAl2021} \\

        5D
        & High gas consumption function type \cite{Rameder2022} \citeA{ ChenEtAl2022}
        & Functions not used in the contract but declared public instead of external require more gas on deployment than necessary.
        & Function declaration public instead of external \cite{Rameder2022}\\

        5E 
        & Under-priced opcodes \cite{Rameder2022}
        & Contracts executing numerous underpriced opcodes may consume substantial computing resources without corresponding gas costs. This mismatch can lead to Denial of Service (DoS) attacks, as high resource consumption can disrupt normal contract operations and impact network performance.
        & \\

        5F
        & Transfer of all the gas \cite{Rameder2022}
        & Solidity provides three built-in functions for transferring ether: transfer(x), send(x), and call(x). Both transfer(x) and send(x) send 2300 gas units along with the ether, sufficient to process the transaction. The call() function, which is recommended, does not specify the amount of gas directly, transferring all available gas to the recipient.
        & \\

        \midrule
        \multicolumn{4}{l}{\textbf{6 - Authentication \& Access Control Vulnerabilities}}\\
        \midrule

        6A
        & Prodigal contract
        & Using msg.sender for transactions might be incorrect in cases where a contract invokes another to refund funds to a specified address. For example, if refunds are meant for an address passed as a parameter, using msg.sender could send funds to the caller contract instead. Additionally, if the recipient address is arbitrary, it might be an ineligible contract. To address these issues, validate transfer addresses by ensuring they are eligible, and avoid using tx.origin for authentication. Use msg.sender only when no recipient address is specified in parameters.
        & \\

        6A1
        & Authorization via transaction origin \cite{Rameder2022}
        & Using tx.origin for authentication instead of the immediate caller's address (msg.sender) can expose a contract to vulnerabilities. Contracts in the call chain between tx.origin and the vulnerable contract could gain unauthorized access to the contract’s assets.
        & Authentication through tx.origin \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, Staderini2022, AgarwalEtAl2022, ZhouEtAl2022, KushwahaEtAl2022a},
        Transaction state dependency \citeA{MunirAndTaha2023},
        Transaction origin use \citeA{ChoiEtAl2021} \\

        6B
        & Unauthorized accessibility due to wrong function or state variable visibility \cite{Rameder2022}
        & In Solidity, inadvertently declaring functions as public or external can expose entry points that may lead to unauthorized access by malicious users.
        & Visibility of exposed functions \cite{Rameder2022} \citeA{ Staderini2022}
        Function or state variable default visibility \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Function/State visibility error \citeA{ChaliasosEtAl2024},
        Unspecified visibility level \citeA{MunirAndTaha2023},
        Bad visibility \citeA{AgarwalEtAl2022},
        Default visibility \citeA{ZhouEtAl2022},
        No restricted write, Implicit visibility level, Non-public variables accessed by public/external functions, Default/Unintended/Erroneous visibility \cite{Rameder2022} \\

        6B1
        & Function default visibility \citeA{WeiEtAl2023, KushwahaEtAl2022a}
        & In solidity, visibility specifiers are used to make functions external, public, internal, or private. Incorrect use of these visibility specifiers can make smart contracts vulnerable and attract attackers.
        & \\
        
        6B2
        & State variable default visibility \citeA{WeiEtAl2023}
        & In Solidity, the default visibility of state variables is internal. This means that if a state variable is not explicitly declared as public or private, it can be accessed and modified only within the contract and derived contracts.
        & \\

        6C
        & Access Control management\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Functions that are supposed to be executed by only users with specific roles are not protected. Therefore, any user can execute them. For example, functions that perform withdrawals or execute dangerous functions like self-destruct should be protected and executed by users with the right permission.
        & \\
        
        6C1
        & Unprotected self-destruction \cite{Rameder2022} \citeA{ ChuEtAl2023, AgarwalEtAl2022, KushwahaEtAl2022a, KushwahaEtAl2022b, Staderini2022, ZhouEtAl2022}
        & Insufficient access control for a SELFDESTRUCT instruction can lead to accidental or malicious contract destruction.
        & Unexpected kill, Destroyable contract \cite{Rameder2022},
        Suicidal contract \citeA{ChoiEtAl2021},
        Unsafe suicide \citeA{WeiEtAl2023},
        Check on suicide functionality \citeA{DiasEtAl2021}\\

        6C2
        & Unauthorized Ether withdrawal \cite{Rameder2022}
        & Insufficient access control on a contract's withdrawal functionality can lead to unauthorized asset theft.
        & Unprotected Ether withdrawal \citeA{Staderini2022, WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, KushwahaEtAl2022a}
        Check on balance withdrawal \citeA{DiasEtAl2021},
        Ether leak \citeA{ChoiEtAl2021} \\

        6D
        & Signature based vulnerabilities \cite{Rameder2022}
        & This vulnerability includes issues like missing protection against signature replay attacks, lack of proper signature verification, hash collisions with multiple variable length arguments, signature malleability, signatures with a wrong parameter, and any related vulnerabilities.
        & Insufficient signature information \cite{Rameder2022} \\

        6D1
        & Missing protection against signature replay attack \cite{Rameder2022} \citeA{ Staderini2022, WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Signature verification in smart contracts can enhance usability or reduce gas costs. By maintaining a list of processed message hashes and only allowing new hashes, developers can prevent the reuse of the same message hash by different users. Vulnerabilities 6D1 and 6D5 may appear similar, but in 6D5, an attacker creates a valid signature with different information to bypass verification, while 6D1 concerns replaying an existing, already executed transaction.
        & \\

        6D2
        & Lack of proper signature verification \cite{Rameder2022} \citeA{ WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Smart contract systems often allow users to sign messages off-chain for flexibility and ease. However, smart contracts must verify the authenticity of these signed messages before processing them, as they cannot sign messages themselves. Some verification systems assume a signed message's authenticity based on msg.sender, which can be problematic in scenarios involving transaction relays through proxies, potentially leading to vulnerabilities.
        & \\

        6D3
        & Hash collision with multiple variable length arguments \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, KushwahaEtAl2022a}
        & Hash collisions can occur when using abi.encodePacked() with parameters of different lengths. Since abi.encodePacked() packs items in order, regardless of array boundaries, an attacker might exploit this by rearranging components in a prior function call to evade signature verification and bypass permissions.
        & \\

        6D4
        & Function Clashing \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Calling a function involves sending a function hash in the transaction's data field, which the EVM uses to determine which function to execute. Due to the weak nature of this hash, collisions are likely. This vulnerability can lead to unintended function execution, potentially resulting in financial losses.
        & \\

        6D5
        & Signature Malleability \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, WeiEtAl2023}
        & In Ethereum, cryptographic signatures are often assumed unique but can be altered without private key access and remain valid. The ecrecover contract allows slight modifications to signature values (v, r, s), which can make contract-level signature verification vulnerable to replay attacks using previously signed messages.
        & \\

        6D6
        & Map overlap \citeA{MunirAndTaha2023}
        & In Solidity, using multiple map data structures can lead to a vulnerability known as "map overlap." This occurs when the sha3 function produces the same hash value for different memory locations across maps, potentially causing collisions. For example, an attacker might exploit this by registering addresses in different maps (e.g., admins and regular users) to bypass authorization.
        & \\

        6E
        & Identity verification \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & This vulnerability happens when the smart contract tries to verify if the caller is a wallet or a smart contract based on its code size. Unfortunately, this can be bypassed by calling the vulnerable contract in the constructor of the smart contract attacker, as the source code of the smart contract while executing the constructor is still 0.
        & \\
        
        \midrule
        \multicolumn{4}{l}{\textbf{7 - Arithmetic bugs}}\\
        \midrule

        7A
        & Integer over- or underflow \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, Staderini2022, KushwahaEtAl2022a, AgarwalEtAl2022, ChuEtAl2023, MunirAndTaha2023}
        & Integer overflow and underflows occur when arithmetic operations exceed the maximum or minimum of integer types.
        & Arithmetic UnderflowOverflow \citeA{KushwahaEtAl2022b},
        Integer bug \citeA{ChoiEtAl2021},
        Value assignment with too many digits \citeA{DiasEtAl2021} \\

        7B
        & Floating point \& Precision \cite{Rameder2022}
        & Handling floating-point numbers as integers can lead to inaccuracies, errors, and vulnerabilities. 
        & \\

        7B1
        & Integer division \cite{Rameder2022}
        & Solidity does not admit floating-point or decimal types and integer division is always rounded toward zero. This choice of rounding method can produce results other than what some users might expect.
        & Money leak \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Unexpected result from division \citeA{MunirAndTaha2023} \\

        7B2
        & Arithmetic Precision \citeA{Staderini2022}
        & Solidity supports integers and (partially) fixed-point numbers. So, integers must be used to represent floating points. The 256-bit EVM assembles types shorter than 32 bytes together in the 32-byte slot affecting the accuracy of any operation; for example, rounding is incorrect if a division is performed before multiplication. 
        & \\
    
        7C
        & Integer bugs or Arithmetic Issues \cite{Rameder2022}
        & Conversion or arithmetic operation between signed and unsigned integers, or between integers of different lengths, can lead to incorrect results.
        & Integer sign \cite{Rameder2022} \citeA{ DiasEtAl2021},
        Signedness bugs \citeA{AgarwalEtAl2022},
        Check on arithmetic operation \citeA{DiasEtAl2021},
        Integer Truncation \cite{Rameder2022} \citeA{ DiasEtAl2021}, Truncation Bugs \citeA{AgarwalEtAl2022},
        Unchecked Math, Wrong operator \cite{Rameder2022}\\

        7C1
        & Unchecked division \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        & Vulnerable code to a non-checked division, like dividing by zero.
        & \\

        \midrule
        \multicolumn{4}{l}{\textbf{8 - Bad Coding Quality and Programming Language Specifics}}\\
        \midrule
        
        8A
        & Type cast \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022}
        & When interacting with another contract, specifying its interface allows the Solidity compiler to construct low-level calls, but the compiler cannot verify if the interface matches the actual contract. Using an incorrect interface specification can invoke unintended entry points and misinterpret arguments, leading to unexpected behavior.
        & Unsafe type declaration, Insecure inference \citeA{MunirAndTaha2023},
        Unsafe type inference \cite{Rameder2022}, Type conversion \citeA{VivarEtAl2021} \\

        8B
        & Coding error \cite{Rameder2022}
        & Coding errors, including typos and other developer errors. 
        & Typographical error \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}, Immutable bugs \cite{Rameder2022} \citeA{ VivarEtAl2021}, Coding Bug\cite{Rameder2022} \\

        8C
        & Bad coding pattern \cite{Rameder2022}
        & Use of various coding patterns that are considered as bad style.
        & \\

        8D
        & Deprecated source language features \cite{Rameder2022}
        & The use of deprecated language features is discouraged, as it may lead to known errors and vulnerabilities that were the cause for deprecation.
        & Use of deprecated Solidity function \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} \\

        8E
        & Write to arbitrary storage location \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, DiasEtAl2021}
        & In Solidity, due to language quirks and programming errors, attackers may modify arbitrary storage locations, such as access control variables. Complex data types like structs, maps, and arrays are statically allocated in storage. Accessing an uninitialized local variable of such types may inadvertently expose the first storage cell.
        & Arbitrary send \citeA{AgarwalEtAl2022},
        Arbitrary write \citeA{ChoiEtAl2021} \\

        8F
        & Use of assembly \cite{Rameder2022} \citeA{ AgarwalEtAl2022}
        & The use of assembly instructions in high-level code is discouraged, as it can lead to various critical vulnerabilities.
        & Assembly-based vulnerabilities \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Usage of assembly\citeA{AgarwalEtAl2022}\\

        8F1
        & Arbitrary jump with function type variable \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}
        & Solidity supports function types, allowing function references with matching signatures to be assigned to variables of that type. If developers use assembly instructions like mstore or the assignment operator improperly, attackers might redirect function type variables to malicious code, bypassing validations and altering state changes.
        & Arbitrary jump \citeA{Staderini2022}, Control-Flow hijack \citeA{ChoiEtAl2021}, Function type variables assignment using arbitrary values \citeA{DiasEtAl2021}, Specify function variable as any type\cite{Rameder2022} \\

        8F2
        & Constant function using assembly code \citeA{AgarwalEtAl2022}
        & Before Solidity 0.5, functions declared as constant, pure, or view could execute assembly code that modified state. Since Solidity 0.5, the STATICCALL opcode is used for constant, pure, and view functions, ensuring that calls revert if state modifications are attempted. 
        & Constant Function \citeA{AgarwalEtAl2022} \\

        8F3
        & Returning results using assembly code in constructor \cite{Rameder2022}
        & The use of assembly within a Solidity constructor to manipulate the contract's deployment process can significantly alter the deployed bytecode from what is expected based on the source code. This approach exploits the flexibility of the EVM to execute low-level operations that bypass standard compilation and deployment procedures.
        & \\
        
        8G
        & Incorrect inheritance order \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}
        & Solidity supports multiple inheritance, which can lead to ambiguity known as the Diamond Problem if multiple base contracts define the same function. This issue is resolved using C3 Linearization, which ensures a deterministic method resolution order. Unawareness of this mechanism can lead to unexpected behavior and vulnerabilities.
        & \\

        8H
        & Variable shadowing \cite{Rameder2022}
        & Solidity allows for ambiguous variable names when inheritance is used, leading to errors and vulnerabilities that are difficult to identify in complex contract systems.
        & Hidden state variable \cite{Rameder2022},
        Shadowing state variables \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Variable name \citeA{DiasEtAl2021},
        Tained memory \citeA{MunirAndTaha2023},
        Shadowing state, Shadowing abstract, Shadowing builtin, Shadowing local \citeA{AgarwalEtAl2022} \\

        8I 
        & Misleading source code \cite{Rameder2022}
        & Malicious actors may apply various strategies to confuse or hide malicious contract code behavior and trick users.
        & API inconsistency \cite{Rameder2022} \\

        8I1
        & Right to Left override \citeA{Staderini2022, WeiEtAl2023} \cite{Rameder2022}
        & The Right-To-Left Override (U+202E) Unicode character allows right-to-left characters in left-to-right text. In smart contracts, inserting RTL characters can covertly alter code behavior, potentially modifying contract logic without users realizing it.
        & \\

        8I2
        & Misleading data location \citeA{ChenEtAl2022}
        & Do not clarify the reference types of local variables of struct, array, or mapping.\citeA{ChenEtAl2022} 
        & \\

        8I3
        & Hidden built-in symbols \cite{Rameder2022}
        & Using built-in symbols in Solidity can alter the default behavior of the language and introduce business logic bugs in smart contracts.
        & Built-in symbol shadowing \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Use of deprecated built-in symbols \citeA{DiasEtAl2021} \\

        8J
        & Missing logic \cite{Rameder2022} 
        & Missing logic, logical errors, or dead code can confuse or lead to unwanted behavior and vulnerabilities.
        & Code with no effects \cite{Rameder2022} \citeA{ WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Presence of unused variables \cite{Rameder2022} \citeA{ WeiEtAl2023},
        Unused statement \citeA{ChenEtAl2022},
        Unused return \citeA{AgarwalEtAl2022},
        Logical errors or dead code \cite{Rameder2022}\\

        8K
        & Insecure contract upgrading \cite{Rameder2022}
        & Upgrading contracts can fix vulnerabilities but contends the goal of complete decentralization. If a developer turns malicious or is compromised, updates may introduce malicious changes. 
        & Upgradable contract, Patching \cite{Rameder2022} \\

        8L 
        & Inadequate or incorrect logging or documentation \cite{Rameder2022}
        & Inadequate logging and documentation can confuse, lead to logical errors or unexpected behavior, and hamper auditing or testing the code for vulnerabilities.
        & \\

        8M
        & Hardcoded addresses \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022, ChenEtAl2022}
        & Using a hard-coded address could make the smart contract useless in the future if one of those addresses changes.
        & \\

        8N
        & Send to zero address \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & This vulnerability happens when the smart contract does not check if the receiver is a Zero address.
        & \\

        8O
        & Double constructor \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Before introducing the constructor keyword in the 0.4.22 version, if a contract declares the constructor using a function with the same name as the contract and also defines a regular function with the same name but a different signature, it can create ambiguity. The compiler identifies constructors by name, leading to potential confusion. An attacker might exploit this by deploying the contract and calling the regular function, potentially causing security issues.
        & \\
        

        \midrule
        \multicolumn{4}{l}{\textbf{9 - Environment Configuration Issues}}\\
        \midrule

        9A
        & Short address \cite{Rameder2022} \citeA{ ZhouEtAl2022, ChuEtAl2023, Staderini2022}
        & The EVM pads addresses with zeroes if they are shorter than required. Addresses with trailing zeroes can be exploited by attackers if client-side sanitation checks are insufficient. 
        & Check on input address length \citeA{DiasEtAl2021},
        Address shortening \citeA{MunirAndTaha2023} \\
        
        9B
        & Outdated compiler version \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}
        & Using outdated compiler versions is strongly discouraged, as old compiler bugs or updates can lead to vulnerabilities in compiled smart contract code.
        & Pragmas version \citeA{AgarwalEtAl2022},
        Unspecified Compiler version \citeA{ChenEtAl2022},
        Compiler version \citeA{DiasEtAl2021} \\

        9C
        & Floating or no pragma \cite{Rameder2022} \citeA{ WeiEtAl2023, KushwahaEtAl2022a}
        & To ensure consistency and avoid discrepancies, the same compiler version and flags used for testing should be used for deploying smart contracts. Therefore, the pragma directive should be locked to the correct compiler version.  
        & Floating compiler version \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} \\

        9D
        & Token API violation \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Tokens that deviate from community standards, such as those proposed by OpenZeppelin, may introduce critical vulnerabilities. For example, some tokens' transfer functions incorrectly throw errors instead of returning a boolean. To avoid these issues and ensure compatibility, token contracts should adhere to established standards like ERC20 or ERC721.
        & Token standard incompatibility \cite{Rameder2022}, Unmatched ERC-20 Standard \citeA{ChenEtAl2022} \\

        9D1
        & Improper or missing event handling \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & This vulnerability, often seen in ERC-20 tokens, arises when a transfer function does not emit an event to notify users of the success or failure of the transfer. This flaw impedes error handling and can lead to critical issues in managing token transactions.
        & Missing Reminder\citeA{ChenEtAl2022}, Fake Deposit\citeA{MunirAndTaha2023} \\

        9E
        & Ethereum update incompatibility \cite{Rameder2022}
        & Future Ethereum hard forks may change gas costs for opcodes, potentially disrupting contracts with fixed gas cost assumptions. If future forks increase gas fees, these contracts may fail due to insufficient gas, resulting in out-of-gas exceptions.
        & Failing to accept new deposit, Deposit Acceptance \citeA{MunirAndTaha2023},
        Message call with hardcoded gas amount \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}\\

        9F
        & Configuration error \cite{Rameder2022}
        & Bad configuration of the smart contract application toolchain can lead to errors and vulnerabilities, even if the smart contract itself is correct.
        & \\

        9G
        & Missing Interrupter~\citeA{ChenEtAl2022}
        & The contract lacks a backdoor mechanism for handling emergencies, making it difficult to address critical issues. Implementing the selfdestruct function could be beneficial.
        & \\

        \midrule
        \multicolumn{4}{l}{\textbf{10 - Eliminated/Deprecated syntax}}\\
        \midrule

        10A
        & Callstack depth limit \cite{Rameder2022}
        & Eliminated by Ethereum upgrade (Oct 18, 2016).
        & Stack size limit \cite{Rameder2022}, 
        Limited stack size \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Stack size \citeA{VivarEtAl2021} \\

        10B
        & Uninitialized storage pointer \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023}
        & Eliminated by Solidity compiler, starting version 0.5.0.
        & Uninitialized local/state variable \cite{Rameder2022},
        Uninitialized state variables \citeA{ChuEtAl2023},
        Uninitialized state, Uninitialized storage, Uninitialized local \citeA{AgarwalEtAl2022},
        Initialization of local variables, Initialization of state variables, Initialization of storage pointer, Missing initialization \citeA{DiasEtAl2021} \\

        10C
        & Erroneous constructor name \cite{Rameder2022}
        & Before Solidity 0.4.22, constructors were defined by naming a function the same as the contract. Erroneous naming could result in contracts without a specific initialization code being executed upon deployment.
        & Incorrect constructor name \cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023},
        Constructor name \citeA{DiasEtAl2021}\\

        10D
        & Deprecated APIs \citeA{ChenEtAl2022}
        & Using discarded or unrecommended APIs or instructions.
        & \\
\end{longtable}

\twocolumn

==> tables/half_taxonomy.tex <==
{
\footnotesize
\begin{longtable}{p{0.3cm} p{7.6cm} p{7cm}}
    
    \caption{A Comprehensive List of Vulnerabilities Hierarchical Organized.}
    \label{tab:half_tax}\\
    \toprule
    \textbf{Id} & \textbf{Name} & \textbf{Alternative Names} \\ 
    \midrule
    \endfirsthead
    \multicolumn{3}{c}{{Continued from previous page}} \\
    \toprule
    \textbf{Id} & \textbf{Name} & \textbf{Alternative Names} \\ 
    \midrule
    \endhead
    \midrule
    \multicolumn{3}{r}{{Continued on next page}} \\
    \midrule
    \endfoot
    \bottomrule
    \endlastfoot

    \multicolumn{3}{l}{\textbf{1 - Malicious Environment, Transactions, or Input}}\\
    \midrule
    
        1A
        & Call to the unknown~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, KushwahaEtAl2022a}
        & Unexpected fallback function~\citeB{Rameder2022} \\
        1A1
        & Reentrancy~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, ChoiEtAl2021, ChuEtAl2023, ZhouEtAl2022, KushwahaEtAl2022b, Staderini2022, ChaliasosEtAl2024}
        & Reentrancy-eth~\citeA{AgarwalEtAl2022}~\citeB{slither}, Cross function race condition, Recursive call vulnerability, Race to empty~\citeB{Rameder2022}\\
        
        \hdashline[0.5pt/1pt]
        
        1B 
        & Exact balance dependency~\citeB{Rameder2022}
        & Unexpected Ether, Manipulated balance,
        Unexpected Balance~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Unexpected Ether balance~\citeA{MunirAndTaha2023},
        Unprotected Ether Balance~\citeA{Staderini2022}, 
        Balance equality~\citeA{AgarwalEtAl2022},
        Strict Balance Equality~\citeA{ChenEtAl2022}\\
        1B1
        & Forcing Ether to contracts~\citeB{Rameder2022}
        & Check on force to receive balance~\citeA{DiasEtAl2021} \\
        1B2
        & Pre-sent Ether~\citeB{Rameder2022}
        & \\
        
        \hdashline[0.5pt/1pt]
        
        1C 
        & Improper data validation~\citeB{Rameder2022} 
        & Untrustworthy data feeds~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, KushwahaEtAl2022a}\\

        \hdashline[0.5pt/1pt]

        1D 
        & Vulnerable Delegatecall~\citeB{Rameder2022} 
        & Delegate call to Untrusted Callee~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023}, Delegate call to Insecure Contracts~\citeA{ZhouEtAl2022}, Unsafe delegatecall~\citeA{WeiEtAl2023}, check on target address in delegatecall~\citeA{DiasEtAl2021}, Delegate call~\citeA{AgarwalEtAl2022, KushwahaEtAl2022a, KushwahaEtAl2022b} \\

        \midrule
        \multicolumn{3}{l}{\textbf{2 - Blockchain/Environment Dependency}}\\
        \midrule

        2A
        & Block State Dependency~\citeA{ChenEtAl2022, ChoiEtAl2021}
        & Block Info Dependency~\citeA{ChenEtAl2022}\\

        2A1
        & Timestamp dependency~\citeB{Rameder2022}~\citeA{ ChuEtAl2023, ZhouEtAl2022, KushwahaEtAl2022a, KushwahaEtAl2022b, Staderini2022}
        & Time constraints, Time manipulation~\citeB{Rameder2022}, Time restriction~\citeA{VivarEtAl2021}, Block values as a proxy for time~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} \\

        2A2
        & Block number dependency~\citeB{Rameder2022}
        & \\

        2A3
        & Blockhash dependency~\citeB{Rameder2022}
        & Blockhash usage~\citeA{Staderini2022} \\

        \hdashline[0.5pt/1pt]

        2B 
        & Transaction-ordering dependency~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, AgarwalEtAl2022, ZhouEtAl2022, ChuEtAl2023, KushwahaEtAl2022a, KushwahaEtAl2022b}
        & Event-ordering bugs~\citeB{Rameder2022}\\

        2B1
        & Front-running attack~\citeB{Rameder2022}
        & Race condition~\citeB{Rameder2022}\\

        \hdashline[0.5pt/1pt]
        
        2C 
        & Bad random number generation~\citeB{Rameder2022}
        & Generating Randomness~\citeB{Rameder2022}~\citeA{ ZhouEtAl2022, Staderini2022},
        Bad randomness~\citeB{Rameder2022},
        Weak Sources of Randomness from Chain Attributes~\citeA{dZaazaaAndElBakkali2023a,dZaazaaAndElBakkali2023b}, Random Number~\citeA{VivarEtAl2021}\\

        2C1
        & Randomness Using Block Hash~\citeA{KushwahaEtAl2022a}
        & \\

        \hdashline[0.5pt/1pt]
        
        2D 
        & Leakage of confidential information~\citeB{Rameder2022} 
        & Lack of transaction privacy~\citeB{Rameder2022}~\citeA{ KushwahaEtAl2022a},
        Private information leakage, Nothing is secret, Confidentiality failure, Keeping secrets, Data exposure~\citeB{Rameder2022},
        On-chain oracle manipulation~\citeA{ChaliasosEtAl2024}, Secrecy failure~\citeA{Staderini2022}, Exposed secret~\citeA{MunirAndTaha2023}, Unencrypted private data on-chain~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}, Secrets~\citeA{VivarEtAl2021} \\

        \hdashline[0.5pt/1pt]
    
        2E
        & Unpredictable state~\citeB{Rameder2022}~\citeA{ VivarEtAl2021}
        & \\

        2E1
        & Dynamic Library~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\

        2E2
        & References to destroyed contracts~\citeA{MunirAndTaha2023}
        & \\

        2E3
        & Using components with known vulnerabilities~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\

        2E4
        & External Contract Referencing~\citeA{ZhouEtAl2022}
        & Misuse of address parameters in the constructor~\citeA{MunirAndTaha2023}, Value assigned to contract address~\citeA{DiasEtAl2021}\\

        \midrule
        \multicolumn{3}{l}{\textbf{3 - Exception \& Error Handling Disorders}}\\
        \midrule
        
        3A
        & Unchecked low-level call/send return values~\citeB{Rameder2022}
        & Unchecked call return values~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022, Staderini2022},
        Unchecked external calls~\citeA{ChenEtAl2022},
        Check on external call~\citeA{MunirAndTaha2023},
        Unchecked call~\citeA{KushwahaEtAl2022b},
        Unchecked send~\citeB{Rameder2022}~\citeA{ Staderini2022, WeiEtAl2023},
        Unhandled exception~\citeB{Rameder2022}~\citeA{ ChuEtAl2023},
        Improper handling of exceptions~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Unchecked/unsafe send~\citeB{Rameder2022}\\

        3A1
        & Send instead of transfer~\citeB{Rameder2022}~\citeA{ MunirAndTaha2023}
        & \\

        \hdashline[0.5pt/1pt]
        
        3B
        & Unexpected throw or revert~\citeB{Rameder2022}
        & Unexpected-throw-DoS, DoS with unexpected revert/throw\citeB{Rameder2022}, DoS with failed call~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023, KushwahaEtAl2022a}, Dos by External contracts~\citeB{Rameder2022}~\citeA{ Staderini2022} \\

        3B1
        & Mishandled out-of-gas exception~\citeB{Rameder2022}
        & Gasless send\citeB{Rameder2022}~\citeA{ Staderini2022, KushwahaEtAl2022a}\\

        \hdashline[0.5pt/1pt]

        3C
        & Assert, require or revert violation~\citeB{Rameder2022}
        & Assert violation~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Assertion failure~\citeA{ChoiEtAl2021},
        Requirement violation~\citeA{ChoiEtAl2021, WeiEtAl2023, Staderini2022},
        Requirement violation by the called smart contract~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Require on input variable~\citeA{DiasEtAl2021},
        Revert require, Exception state~\citeA{AgarwalEtAl2022}\\

        \midrule
        \multicolumn{3}{l}{\textbf{4 - Denial of Service}}\\
        \midrule

        4A
        & Greedy contract~\citeB{Rameder2022}
        & Locked Ether~\citeB{Rameder2022},
        Freezing Ether~\citeA{Staderini2022, ZhouEtAl2022, ChoiEtAl2021, KushwahaEtAl2022b}\\

        4A1
        & Locked Money~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022, ChuEtAl2023} 
        & \\

        4A2
        & Frozen Ether~\citeB{Rameder2022}
        & \\

        \hdashline[0.5pt/1pt]

        4B
        & Ether lost in transfer\citeB{Rameder2022} 
        & Transfer to orphan address~\citeB{Rameder2022},
        Lost of Ether~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, KushwahaEtAl2022a}, Loss of Ether~\citeA{VivarEtAl2021}\\

        \hdashline[0.5pt/1pt]

        4C
        & DoS with block gas limit reached~\citeB{Rameder2022}~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, KushwahaEtAl2022a}
        & DoS Costly Pattern and Loops~\citeA{Staderini2022},
        Check on gas Limit~\citeA{DiasEtAl2021},
        Gas limit in loops, Extra Gas in loop~\citeA{AgarwalEtAl2022} \\

        4C1
        & Multiple calls in a single transaction~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Nested Call~\citeA{ChenEtAl2022}, Multiple calls, Transfer in loop~\citeA{AgarwalEtAl2022}\\
        
        4C2
        & Array length manipulation~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022}
        & \\
        
        4C3
        & Infinite loop~\citeA{WeiEtAl2023}
        & Unbounded mass operation~\citeA{MunirAndTaha2023} \\

        \hdashline[0.5pt/1pt]
        
        4D
        & DoS by Exception inside loop~\citeB{Rameder2022}
        & DoS under external influence~\citeB{Rameder2022}~\citeA{ ChenEtAl2022}, Wallet griefing causing out of gas exception~\citeB{Rameder2022} \\

        \hdashline[0.5pt/1pt]

        4E
        & Insufficient gas griefing~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023, WeiEtAl2023, KushwahaEtAl2022a}
        & \\

        \hdashline[0.5pt/1pt]

        4F
        & Overpowered Role~\citeA{AgarwalEtAl2022}
        & Check on overpowered role~\citeA{DiasEtAl2021} \\

        \hdashline[0.5pt/1pt]

        4G
        & Missed to implement a fallback function~\citeA{MunirAndTaha2023}
        & \\
        
        \midrule
        \multicolumn{3}{l}{\textbf{5 - Resurce Consuption \& Gas Related Issues}}\\
        \midrule

        5A 
        & Gas costly loops~\citeB{Rameder2022} 
        & Invariants in loops~\citeB{Rameder2022} \\

        \hdashline[0.5pt/1pt]

        5B
        & Gas costly pattern~\citeB{Rameder2022}
        & \\

        \hdashline[0.5pt/1pt]

        5C
        & High gas consumption of variable data type or declaration
        & \\

        5C1
        & Byte Array~\citeB{Rameder2022}
        & Variable type~\citeA{DiasEtAl2021}\\

        5C2
        & Invariant State variables not declared constant~\citeB{Rameder2022} 
        & Declaration of invariant state variable~\citeA{DiasEtAl2021} \\

        \hdashline[0.5pt/1pt]

        5D
        & High gas consumption function type~\citeB{Rameder2022}~\citeA{ ChenEtAl2022}
        & Function declaration public instead of external~\citeB{Rameder2022}\\

        \hdashline[0.5pt/1pt]

        5E 
        & Under-priced opcodes~\citeB{Rameder2022}
        & \\

        \hdashline[0.5pt/1pt]

        5F
        & Transfer of all the gas~\citeB{Rameder2022}
        & \\

        \midrule
        \multicolumn{3}{l}{\textbf{6 - Authentication \& Access Control Vulnerabilities}}\\
        \midrule

        6A
        & Prodigal contract
        & \\

        6A1
        & Authorization via transaction origin~\citeB{Rameder2022}
        & Authentication through tx.origin~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, Staderini2022, AgarwalEtAl2022, ZhouEtAl2022, KushwahaEtAl2022a},
        Transaction state dependency~\citeA{MunirAndTaha2023},
        Transaction origin use~\citeA{ChoiEtAl2021} \\

        \hdashline[0.5pt/1pt]

        6B
        & Unauthorized accessibility due to wrong function or state variable visibility~\citeB{Rameder2022}
        & Visibility of exposed functions~\citeB{Rameder2022}~\citeA{ Staderini2022}
        Function or state variable default visibility~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Function/State visibility error~\citeA{ChaliasosEtAl2024},
        Unspecified visibility level~\citeA{MunirAndTaha2023},
        Bad visibility~\citeA{AgarwalEtAl2022},
        Default visibility~\citeA{ZhouEtAl2022},
        No restricted write, Implicit visibility level, Non-public variables accessed by public/external functions, Default/Unintended/Erroneous visibility~\citeB{Rameder2022} \\

        6B1
        & Function default visibility~\citeA{WeiEtAl2023, KushwahaEtAl2022a}
        & \\
        
        6B2
        & State variable default visibility~\citeA{WeiEtAl2023}
        & \\

        \hdashline[0.5pt/1pt]

        6C
        & Access Control management~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\
        
        6C1
        & Unprotected self-destruction~\citeB{Rameder2022}~\citeA{ ChuEtAl2023, AgarwalEtAl2022, KushwahaEtAl2022a, KushwahaEtAl2022b, Staderini2022, ZhouEtAl2022}
        & Unexpected kill, Destroyable contract~\citeB{Rameder2022},
        Suicidal contract~\citeA{ChoiEtAl2021},
        Unsafe suicide~\citeA{WeiEtAl2023},
        Check on suicide functionality~\citeA{DiasEtAl2021}\\

        6C2
        & Unauthorized Ether withdrawal~\citeB{Rameder2022}
        & Unprotected Ether withdrawal~\citeA{Staderini2022, WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, KushwahaEtAl2022a}
        Check on balance withdrawal~\citeA{DiasEtAl2021},
        Ether leak~\citeA{ChoiEtAl2021} \\

        \hdashline[0.5pt/1pt]

        6D
        & Signature based vulnerabilities~\citeB{Rameder2022}
        & Insufficient signature information~\citeB{Rameder2022} \\

        6D1
        & Missing protection against signature replay attack~\citeB{Rameder2022}~\citeA{ Staderini2022, WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\

        6D2
        & Lack of proper signature verification~\citeB{Rameder2022}~\citeA{ WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\

        6D3
        & Hash collision with multiple variable length arguments~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, KushwahaEtAl2022a}
        & \\

        6D4
        & Function Clashing~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\

        6D5
        & Signature Malleability~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, WeiEtAl2023}
        & \\

        6D6
        & Map overlap~\citeA{MunirAndTaha2023}
        & \\

        \hdashline[0.5pt/1pt]

        6E
        & Identity verification~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\
        
        \midrule
        \multicolumn{3}{l}{\textbf{7 - Arithmetic bugs}}\\
        \midrule

        7A
        & Integer over- or underflow~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, Staderini2022, KushwahaEtAl2022a, AgarwalEtAl2022, ChuEtAl2023, MunirAndTaha2023}
        & Arithmetic UnderflowOverflow~\citeA{KushwahaEtAl2022b},
        Integer bug~\citeA{ChoiEtAl2021},
        Value assignment with too many digits~\citeA{DiasEtAl2021} \\

        \hdashline[0.5pt/1pt]

        7B
        & Floating point \& Precision~\citeB{Rameder2022}
        & \\

        7B1
        & Integer division~\citeB{Rameder2022}
        & Money leak~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Unexpected result from division~\citeA{MunirAndTaha2023} \\

        7B2
        & Arithmetic Precision~\citeA{Staderini2022}
        & \\

        \hdashline[0.5pt/1pt]
    
        7C
        & Integer bugs or Arithmetic Issues~\citeB{Rameder2022}
        & Integer sign~\citeB{Rameder2022}~\citeA{ DiasEtAl2021},
        Signedness bugs~\citeA{AgarwalEtAl2022},
        Check on arithmetic operation~\citeA{DiasEtAl2021},
        Integer Truncation~\citeB{Rameder2022}~\citeA{ DiasEtAl2021}, Truncation Bugs~\citeA{AgarwalEtAl2022},
        Unchecked Math, Wrong operator~\citeB{Rameder2022}\\

        7C1
        & Unchecked division~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        & \\

        \midrule
        \multicolumn{3}{l}{\textbf{8 - Bad Coding Quality and Programming Language Specifics}}\\
        \midrule
        
        8A
        & Type cast~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022}
        & Unsafe type declaration, Insecure inference~\citeA{MunirAndTaha2023},
        Unsafe type inference~\citeB{Rameder2022}, Type conversion~\citeA{VivarEtAl2021} \\

        \hdashline[0.5pt/1pt]

        8B
        & Coding error~\citeB{Rameder2022}
        & Typographical error~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}, Immutable bugs~\citeB{Rameder2022}~\citeA{ VivarEtAl2021}, Coding Bug\citeB{Rameder2022} \\

        \hdashline[0.5pt/1pt]

        8C
        & Bad coding pattern~\citeB{Rameder2022}
        & \\

        \hdashline[0.5pt/1pt]

        8D
        & Deprecated source language features~\citeB{Rameder2022}
        & Use of deprecated Solidity function~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} \\

        \hdashline[0.5pt/1pt]

        8E
        & Write to arbitrary storage location~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, DiasEtAl2021}
        & Arbitrary send~\citeA{AgarwalEtAl2022},
        Arbitrary write~\citeA{ChoiEtAl2021} \\

        \hdashline[0.5pt/1pt]

        8F
        & Use of assembly~\citeB{Rameder2022}~\citeA{ AgarwalEtAl2022}
        & Assembly-based vulnerabilities~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Usage of assembly~\citeA{AgarwalEtAl2022}\\

        8F1
        & Arbitrary jump with function type variable~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}
        & Arbitrary jump~\citeA{Staderini2022}, Control-Flow hijack~\citeA{ChoiEtAl2021}, Function type variables assignment using arbitrary values~\citeA{DiasEtAl2021}, Specify function variable as any type\citeB{Rameder2022} \\

        8F2
        & Constant function using assembly code~\citeA{AgarwalEtAl2022} 
        & Constant Function~\citeA{AgarwalEtAl2022} \\

        8F3
        & Returning results using assembly code in constructor~\citeB{Rameder2022}
        & \\

        \hdashline[0.5pt/1pt]
        
        8G
        & Incorrect inheritance order~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}
        & \\

        \hdashline[0.5pt/1pt]

        8H
        & Variable shadowing~\citeB{Rameder2022}
        & Hidden state variable~\citeB{Rameder2022},
        Shadowing state variables~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Variable name~\citeA{DiasEtAl2021},
        Tained memory~\citeA{MunirAndTaha2023},
        Shadowing state, Shadowing abstract, Shadowing builtin, Shadowing local~\citeA{AgarwalEtAl2022} \\

        \hdashline[0.5pt/1pt]

        8I 
        & Misleading source code~\citeB{Rameder2022}
        & API inconsistency~\citeB{Rameder2022} \\

        8I1
        & Right to Left override~\citeA{Staderini2022, WeiEtAl2023}~\citeB{Rameder2022}
        & \\

        8I2
        & Misleading data location~\citeA{ChenEtAl2022}
        & \\

        8I3
        & Hidden built-in symbols~\citeB{Rameder2022}
        & Built-in symbol shadowing~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Use of deprecated built-in symbols~\citeA{DiasEtAl2021} \\

        \hdashline[0.5pt/1pt]

        8J
        & Missing logic~\citeB{Rameder2022} 
        & Code with no effects~\citeB{Rameder2022}~\citeA{ WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Presence of unused variables~\citeB{Rameder2022}~\citeA{ WeiEtAl2023},
        Unused statement~\citeA{ChenEtAl2022},
        Unused return~\citeA{AgarwalEtAl2022},
        Logical errors or dead code~\citeB{Rameder2022}\\

        \hdashline[0.5pt/1pt]

        8K
        & Insecure contract upgrading~\citeB{Rameder2022}
        & Upgradable contract, Patching~\citeB{Rameder2022} \\

        \hdashline[0.5pt/1pt]

        8L 
        & Inadequate or incorrect logging or documentation~\citeB{Rameder2022}
        & \\

        \hdashline[0.5pt/1pt]

        8M
        & Hardcoded addresses~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022, ChenEtAl2022}
        & \\

        \hdashline[0.5pt/1pt]

        8N
        & Send to zero address~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\

        \hdashline[0.5pt/1pt]

        8O
        & Double constructor~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\

        \midrule
        \multicolumn{3}{l}{\textbf{9 - Environment Configuration Issues}}\\
        \midrule

        9A
        & Short address~\citeB{Rameder2022}~\citeA{ ZhouEtAl2022, ChuEtAl2023, Staderini2022}
        & Check on input address length~\citeA{DiasEtAl2021},
        Address shortening~\citeA{MunirAndTaha2023} \\

        \hdashline[0.5pt/1pt]
        
        9B
        & Outdated compiler version~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}
        & Pragmas version~\citeA{AgarwalEtAl2022},
        Unspecified Compiler version~\citeA{ChenEtAl2022},
        Compiler version~\citeA{DiasEtAl2021} \\

        \hdashline[0.5pt/1pt]

        9C
        & Floating or no pragma~\citeB{Rameder2022}~\citeA{ WeiEtAl2023, KushwahaEtAl2022a}
        & Floating compiler version~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} \\

        \hdashline[0.5pt/1pt]

        9D
        & Token API violation~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Token standard incompatibility~\citeB{Rameder2022}, Unmatched ERC-20 Standard~\citeA{ChenEtAl2022} \\

        9D1
        & Improper or missing event handling~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Missing Reminder~\citeA{ChenEtAl2022}, Fake Deposit~\citeA{MunirAndTaha2023} \\

        \hdashline[0.5pt/1pt]

        9E
        & Ethereum update incompatibility~\citeB{Rameder2022}
        & Failing to accept new deposit, Deposit Acceptance~\citeA{MunirAndTaha2023},
        Message call with hardcoded gas amount~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}\\

        \hdashline[0.5pt/1pt]

        9F
        & Configuration error~\citeB{Rameder2022}
        & \\

        \hdashline[0.5pt/1pt]

        9G
        & Missing Interrupter~\citeA{ChenEtAl2022}
        & \\

        \midrule
        \multicolumn{3}{l}{\textbf{10 - Eliminated/Deprecated syntax}}\\
        \midrule

        10A
        & Callstack depth limit~\citeB{Rameder2022}
        & Stack size limit~\citeB{Rameder2022}, 
        Limited stack size~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Stack size~\citeA{VivarEtAl2021} \\

        \hdashline[0.5pt/1pt]

        10B
        & Uninitialized storage pointer~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023}
        & Uninitialized local/state variable~\citeB{Rameder2022},
        Uninitialized state variables~\citeA{ChuEtAl2023},
        Uninitialized state, Uninitialized storage, Uninitialized local~\citeA{AgarwalEtAl2022},
        Initialization of local variables, Initialization of state variables, Initialization of storage pointer, Missing initialization~\citeA{DiasEtAl2021} \\

        \hdashline[0.5pt/1pt]

        10C
        & Erroneous constructor name~\citeB{Rameder2022}
        & Incorrect constructor name~\citeB{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023},
        Constructor name~\citeA{DiasEtAl2021}\\

        \hdashline[0.5pt/1pt]

        10D
        & Deprecated APIs~\citeA{ChenEtAl2022}
        & \\
\end{longtable}
}

==> tables/short_taxonomy.tex <==
\begin{center}
\scriptsize

\tablefirsthead{\toprule \textbf{Code} &\multicolumn{1}{c}{\textbf{Vulnerability}} \\ \midrule}

\tablehead{%
    \midrule
    \multicolumn{2}{l}{Continued from previous column} \\
    \toprule
    \textbf{Code} &\multicolumn{1}{c}{\textbf{Vulnerability}} \\ 
    \midrule
}

\tabletail{%
    \midrule 
    \multicolumn{2}{r}{{Continued on next column}}\\
    \midrule
}
    
\tablelasttail{
    \bottomrule
}

\topcaption{Consolidated taxonomy of SCs vulnerability on Ethereum.}
\label{tab:short_tax}

    \begin{supertabular}{p{0.3cm}p{7.8cm}}
        \multicolumn{2}{l}{\textbf{1 - Malicious Environment, Transactions or Input}}\\
        \midrule

    
        1A
        & Call to the unknown~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, KushwahaEtAl2022a}\\

        1A1
        & Reentrancy~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, ChoiEtAl2021, ChuEtAl2023, ZhouEtAl2022, KushwahaEtAl2022b, Staderini2022, ChaliasosEtAl2024}\\
        
        1B 
        & Exact balance dependency~\cite{Rameder2022}\\

        1B1
        & Forcing Ether to contracts~\cite{Rameder2022}
        \\
        1B2
        & Pre-sent Ether~\cite{Rameder2022}\\
        
        1C 
        & Improper data validation~\cite{Rameder2022} \\

        1D 
        & Vulnerable Delegatecall~\cite{Rameder2022} \\

        \midrule
        \multicolumn{2}{l}{\textbf{2 - Blockchain/Environment Dependency}}\\
        \midrule

        2A
        & Block State Dependency~\citeA{ChenEtAl2022, ChoiEtAl2021}\\

        2A1
        & Timestamp dependency~\cite{Rameder2022} \citeA{ ChuEtAl2023, ZhouEtAl2022, KushwahaEtAl2022a, KushwahaEtAl2022b, Staderini2022}\\

        2A2
        & Block number dependency~\cite{Rameder2022}\\

        2A3
        & Blockhash dependency~\cite{Rameder2022}\\

        2B 
        & Transaction-ordering dependency~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, AgarwalEtAl2022, ZhouEtAl2022, ChuEtAl2023, KushwahaEtAl2022a, KushwahaEtAl2022b}\\

        2B1
        & Front-running attack~\cite{Rameder2022}\\
        
        2C 
        & Bad random number generation~\cite{Rameder2022}\\

        2C1
        & Randomness Using Block Hash~\citeA{KushwahaEtAl2022a}\\
        
        2D 
        & Leakage of confidential information~\cite{Rameder2022} \\
    
        2E
        & Unpredictable state~\cite{Rameder2022} \citeA{ VivarEtAl2021}\\

        2E1
        & Dynamic Library~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}\\

        2E2
        & References to destroyed contracts~\citeA{MunirAndTaha2023}\\

        2E3
        & Using components with known vulnerabilities\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} \\

        2E4
        & External Contract Referencing~\citeA{ZhouEtAl2022}\\

        \midrule
        \multicolumn{2}{l}{\textbf{3 - Exception \& Error Handling Disorders}}\\
        \midrule
        
        3A
        & Unchecked low-level call/send return values~\cite{Rameder2022}\\

        3A1
        & Send instead of transfer~\cite{Rameder2022} \citeA{ MunirAndTaha2023}\\
        
        3B
        & Unexpected throw or revert~\cite{Rameder2022}\\

        3B1
        & Mishandled out-of-gas exception~\cite{Rameder2022}\\

        3C
        & Assert, require or revert violation~\cite{Rameder2022}\\

        \midrule
        \multicolumn{2}{l}{\textbf{4 - Denial of Service}}\\
        \midrule

        4A
        & Greedy contract~\cite{Rameder2022}\\

        4A1
        & Locked Money~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022, ChuEtAl2023}\\

        4A2
        & Frozen Ether~\cite{Rameder2022}\\

        4B
        & Ether lost in transfer\cite{Rameder2022}\\

        4C
        & DoS with block gas limit reached~\cite{Rameder2022} \citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, KushwahaEtAl2022a}\\

        4C1
        & Multiple calls in a single transaction~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}\\
        
        4C2
        & Array length manipulation~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022}\\
        
        4C3
        & Infinite loop~\citeA{WeiEtAl2023}\\
        
        4D
        & DoS by Exception inside loop~\cite{Rameder2022}\\

        4E
        & Insufficient gas griefing~\cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023, WeiEtAl2023, KushwahaEtAl2022a}\\

        4F
        & Overpowered Role~\citeA{AgarwalEtAl2022}\\

        4G
        & Missed to implement a fallback function~\citeA{MunirAndTaha2023}\\
        
        \midrule
        \multicolumn{2}{l}{\textbf{5 - Resurce Consuption \& Gas Related Issues}}\\
        \midrule

        5A 
        & Gas costly loops~\cite{Rameder2022}\\

        5B
        & Gas costly pattern~\cite{Rameder2022}\\

        5C
        & High gas consumption of variable data type or declaration~\cite{Rameder2022}\\

        5C1
        & Byte Array~\cite{Rameder2022}\\

        5C2
        & Invariant State variables not declared constant~\cite{Rameder2022} \\

        5D
        & High gas consumption function type~\cite{Rameder2022} \citeA{ ChenEtAl2022}\\

        5E 
        & Under-priced opcodes~\cite{Rameder2022}\\

        5F
        & Transfer of all the gas~\cite{Rameder2022}\\

        \midrule
        \multicolumn{2}{l}{\textbf{6 - Authentication \& Access Control Vulnerabilities}}\\
        \midrule

        6A
        & Prodigal contract~\citeA{MunirAndTaha2023}\\

        6A1
        & Authorization via transaction origin~\cite{Rameder2022}\\

        6B
        & Unauthorized access due to wrong function or state variable visibility~\cite{Rameder2022}\\

        6B1
        & Function default visibility~\citeA{WeiEtAl2023, KushwahaEtAl2022a}\\
        
        6B2
        & State variable default visibility~\citeA{WeiEtAl2023}\\

        6C
        & Access Control management\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}\\
        
        6C1
        & Unprotected self-destruction~\cite{Rameder2022} \citeA{ ChuEtAl2023, AgarwalEtAl2022, KushwahaEtAl2022a, KushwahaEtAl2022b, Staderini2022, ZhouEtAl2022}\\

        6C2
        & Unauthorized Ether withdrawal~\cite{Rameder2022}\\

        6D
        & Signature based vulnerabilities~\cite{Rameder2022}
         \\

        6D1
        & Missing protection against signature replay attack~\cite{Rameder2022} \citeA{ Staderini2022, WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}\\

        6D2
        & Lack of proper signature verification~\cite{Rameder2022} \citeA{ WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}\\

        6D3
        & Hash collision with multiple variable length arguments~\cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, KushwahaEtAl2022a}\\

        6D4
        & Function Clashing~\cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}\\

        6D5
        & Signature Malleability~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, WeiEtAl2023}\\

        6D6
        & Map overlap~\citeA{MunirAndTaha2023}\\

        6E
        & Identity verification~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}\\
        
        \midrule
        \multicolumn{2}{l}{\textbf{7 - Arithmetic bugs}}\\
        \midrule

        7A
        & Integer over- or underflow~\cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, Staderini2022, KushwahaEtAl2022a, AgarwalEtAl2022, ChuEtAl2023, MunirAndTaha2023} \\

        7B
        & Floating point \& Precision~\cite{Rameder2022}\\

        7B1
        & Integer division~\cite{Rameder2022}\\

        7B2
        & Arithmetic Precision~\citeA{Staderini2022}\\
    
        7C
        & Integer bugs or Arithmetic Issues~\cite{Rameder2022}\\

        7C1
        & Unchecked division~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},\\

        \midrule
        \multicolumn{2}{l}{\textbf{8 - Bad Coding Quality and Programming Language Specifics}}\\
        \midrule
        
        8A
        & Type cast~\cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022}\\

        8B
        & Coding error~\cite{Rameder2022}\\

        8C
        & Bad coding pattern~\cite{Rameder2022}\\

        8D
        & Deprecated source language features~\cite{Rameder2022}\\

        8E
        & Write to arbitrary storage location~\cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, DiasEtAl2021}\\

        8F
        & Use of assembly~\cite{Rameder2022} \citeA{ AgarwalEtAl2022}\\

        8F1
        & Arbitrary jump with function type variable~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}\\

        8F2
        & Constant Function~\citeA{AgarwalEtAl2022}\\

        8F3
        & Returning results using assembly code in constructor~\cite{Rameder2022}\\
        
        8G
        & Incorrect inheritance order~\cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}\\

        8H
        & Variable shadowing~\cite{Rameder2022}\\

        8I 
        & Misleading source code~\cite{Rameder2022}\\

        8I1
        & Right to Left override~\citeA{Staderini2022, WeiEtAl2023}\cite{Rameder2022}\\

        8I2
        & Misleading data location~\citeA{ChenEtAl2022}\\

        8I3
        & Hidden built-in symbols~\cite{Rameder2022}\\

        8J
        & Missing logic~\cite{Rameder2022} \\

        8K
        & Insecure contract upgrading~\cite{Rameder2022}\\

        8L 
        & Inadequate or incorrect logging or documentation~\cite{Rameder2022}\\

        8M
        & Hardcoded addresses~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022, ChenEtAl2022}\\

        8N
        & Send to zero address~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}\\

        8O
        & Double constructor~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}\\
        

        \midrule
        \multicolumn{2}{l}{\textbf{9 - Environment Configuration Issues}}\\
        \midrule

        9A
        & Short address~\cite{Rameder2022} \citeA{ ZhouEtAl2022, ChuEtAl2023, Staderini2022}\\
        
        9B
        & Outdated compiler version~\cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}\\

        9C
        & Floating or no pragma~\cite{Rameder2022} \citeA{ WeiEtAl2023, KushwahaEtAl2022a}\\

        9D
        & Token API violation~\cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}\\

        9D1
        & Improper or missing event handling~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}\\

        9E
        & Ethereum update incompatibility~\cite{Rameder2022}\\

        9F
        & Configuration error~\cite{Rameder2022}\\

        9G
        & Missing Interrupter~\citeA{ChenEtAl2022}\\

        \midrule
        \multicolumn{2}{l}{\textbf{10 - Eliminated/Deprecated syntax}}\\
        \midrule

        10A
        & Callstack depth limit~\cite{Rameder2022}\\

        10B
        & Uninitialized storage pointer~\cite{Rameder2022} \citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023}\\

        10C
        & Erroneous constructor name~\cite{Rameder2022}\\

        10D
        & Deprecated APIs~\citeA{ChenEtAl2022}\\

\end{supertabular}
\end{center}



==> tables/tab_idqXclass.tex <==
\begin{table}[ht]
\footnotesize
\centering
\caption{Distribution of IDQ scores per publication class.}
\label{tab:distr_IDQ_class}
\rowcolors{2}{gray!5}{white}
\begin{tabular}{lccccc}
\toprule
~ & \textbf{0.2} & \textbf{0.4} & \textbf{0.5} & \textbf{0.8} & \textbf{1.0} \\
\midrule
\textbf{SLR}     & 1 & 0 & 2 & 2 & 5  \\
\textbf{Survey}  & 35 & 3 & 6 & 8 & 21  \\
\textbf{PS}      & 37 & 10 & 26 & 33 & 88  \\
\hline
\end{tabular}
\end{table}


==> tables/tab_idqXvenue.tex <==
\begin{table}[ht]
\footnotesize
\centering
\caption{Number of publications per IDQ score, by publication venue.}
\label{tab:distr_IDQ_venue}
\rowcolors{2}{gray!5}{white}
\begin{tabular}{lcccccc}
\toprule
~ & \textbf{Journal} & \textbf{Proceeding} & \textbf{Book Section} & \textbf{Preprint} & \textbf{Thesis/Seminar} & \textbf{Total} \\
\midrule
\textbf{0.2} & 8 & 37 & 3 & 13 & 12 & ~ \\
\textbf{0.4} & 0 & 13 & 0 & 0 & 0 & ~ \\
\textbf{0.5} & 20 & 7 & 7 & 0 & 0 & ~ \\
\textbf{0.8} & 35 & 8 & 0 & 0 & 0 & ~ \\
\textbf{1.0} & 65 & 47 & 1 & 1 & 0 & ~ \\
\hline
\end{tabular}
\end{table}



==> tables/tab_venueXclass.tex <==
\begin{table}[ht]
\footnotesize
\centering
\caption{Distribution of publication venues per publication class.}
\label{tab:distr_venue_class}
\rowcolors{2}{gray!5}{white}
\begin{tabular}{lcccccc}
\toprule
~ & \textbf{Journal} & \textbf{Proceeding} & \textbf{Book Section} & \textbf{Preprint} & \textbf{Thesis/Seminar} & \textbf{Total} \\
\midrule
\textbf{SLR}     & 7  & 2  & 0 & 0 & 1 & ~ \\
\textbf{Survey}  & 28 & 29 & 2 & 6 & 8 & ~ \\
\textbf{PS}      & 93 & 81 & 9 & 8 & 3 & ~ \\
\hline
\end{tabular}
\end{table}

==> tables/taxonomy2.tex <==
{
\tiny
\begin{longtable}{p{0.5cm} p{7.2cm} p{7.3cm}}
    \caption{A Comprehensive List of Vulnerabilities Hierarchically Organized.}
    \label{tab:final_tax}\\
    \toprule
    \textbf{Id} & \textbf{Name} & \textbf{Alternative Names} \\
    \midrule
    \endfirsthead
    \multicolumn{3}{c}{{Continued from previous page}} \\
    \toprule
    \textbf{Id} & \textbf{Name} & \textbf{Alternative Names} \\ 
    \midrule
    \endhead
    \midrule
    \multicolumn{3}{r}{{Continued on next page}} \\
    \midrule
    \endfoot
    \bottomrule
    \endlastfoot

    \multicolumn{3}{l}{\textbf{1 - Malicious Environment, Transactions, or Input}}\\
    \midrule
    
        1A
        & Call to the unknown~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, KushwahaEtAl2022a}
        & Unexpected fallback function~\cite{Rameder2022} \\ 
        1A1
        & Reentrancy~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, ChoiEtAl2021, ChuEtAl2023, ZhouEtAl2022, KushwahaEtAl2022b, Staderini2022, ChaliasosEtAl2024}
        & \bluelink{https://swcregistry.io/docs/SWC-107/}{SWC-107}, \bluelink{https://owasp.org/www-project-smart-contract-top-10/2025/en/src/SC05-reentrancy-attacks.html}{OWASP-SC05}, \bluelink{https://dasp.co/\#item-1}{DASP-1}, Cross function race condition, Recursive call vulnerability, Race to empty~\cite{Rameder2022}\\
        1A1.1
        & Reentrancy with ETH transfer~\citeA{li2024static}
        & Reentrancy-eth~\citeA{AgarwalEtAl2022}~\cite{slither}, Unsafe Credit Transfer~\citeA{vidal2024openscv}\\
        1A1.2
        & Reentrancy without ETH transfer~\citeA{li2024static}
        & Reentrancy-no-eth~\citeA{AgarwalEtAl2022}~\cite{slither}, Unsafe System State Changes~\citeA{vidal2024openscv}\\
        1A1.3
        & Reentrancy with same effect~\citeA{li2024static}
        & Reentrancy benign~\citeA{AgarwalEtAl2022}~\cite{slither}\\
        1A1.4
        & Reentrancy with negative events~\citeA{li2024static}
        & Reentrancy events~\citeA{AgarwalEtAl2022}~\cite{slither}\\
        
        \rowcolor{gray!6}
        1B 
        & Exact balance dependency~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-132/}{SWC-132}, Unexpected Ether, Manipulated balance,
        Unexpected Balance~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Unexpected Ether balance~\citeA{MunirAndTaha2023},
        Unprotected Ether Balance~\citeA{Staderini2022}, 
        Balance equality~\citeA{AgarwalEtAl2022},
        Strict Balance Equality~\citeA{ChenEtAl2022},
        Improper Locking~\citeA{vidal2024openscv}\\ \rowcolor{gray!6}
        1B1
        & Forcing Ether to contracts~\cite{Rameder2022}
        & Check on force to receive balance~\citeA{DiasEtAl2021},
        Force Sending Ether with this.balance check in require() or assert()~\citeA{li2024static}\\ \rowcolor{gray!6}
        1B2
        & Pre-sent Ether~\cite{Rameder2022}
        & \\ 
        
        
        1C 
        & Improper data validation~\cite{Rameder2022} 
        & Untrustworthy data feeds~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, KushwahaEtAl2022a}\\
        
        \rowcolor{gray!6}
        1D 
        & Vulnerable Delegatecall~\cite{Rameder2022} 
        & \bluelink{https://swcregistry.io/docs/SWC-112/}{SWC-112}, Delegatecall to Untrusted Callee~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023, vidal2024openscv}, Delegate call to Insecure Contracts~\citeA{ZhouEtAl2022}, Unsafe delegatecall~\citeA{WeiEtAl2023, li2024static}, check on target address in delegatecall~\citeA{DiasEtAl2021}, Delegate call~\citeA{AgarwalEtAl2022, KushwahaEtAl2022a, KushwahaEtAl2022b} \\

        \midrule
        \multicolumn{3}{l}{\textbf{2 - Blockchain/Environment Dependency}}\\
        \midrule

        2A
        & Block State Dependency~\citeA{ChenEtAl2022, ChoiEtAl2021}
        & Block Info Dependency~\citeA{ChenEtAl2022}\\

        2A1
        & Timestamp dependency~\cite{Rameder2022}~\citeA{ ChuEtAl2023, ZhouEtAl2022, KushwahaEtAl2022a, KushwahaEtAl2022b, Staderini2022}
        & \bluelink{https://swcregistry.io/docs/SWC-116/}{SWC-116}, \bluelink{https://dasp.co/\#item-8}{DASP-8}, Time constraints, Time manipulation~\cite{Rameder2022}, Time restriction~\citeA{VivarEtAl2021}, Block values as a proxy for time~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Incorrect Use of Event Blockchain variables for Time~\citeA{vidal2024openscv}\\

        2A2
        & Block number dependency~\cite{Rameder2022}
        & \\

        2A3
        & Blockhash dependency~\cite{Rameder2022}
        & Blockhash usage~\citeA{Staderini2022} \\

        \rowcolor{gray!6}
        
        2B 
        & Transaction-ordering dependency~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, AgarwalEtAl2022, ZhouEtAl2022, ChuEtAl2023, KushwahaEtAl2022a, KushwahaEtAl2022b}
        & \bluelink{https://swcregistry.io/docs/SWC-114/}{SWC-114}, Event-ordering bugs~\cite{Rameder2022},
        Incorrect Function Call Order~\citeA{vidal2024openscv}, time-of-check vs time-of-use\\
        \rowcolor{gray!6}
        2B1
        & Front-running attack~\cite{Rameder2022}
        & \bluelink{https://dasp.co/\#item-7}{DASP-7}, Race condition~\cite{Rameder2022}\\
        \rowcolor{gray!6}
        2B2
        & Transfer Pre-Condition Dependent on Transaction Order~\citeA{vidal2024openscv}
        & \\
        \rowcolor{gray!6}
        2B3
        & Transfer Amount Depending on Transaction Order~\citeA{vidal2024openscv}
        & \\
        \rowcolor{gray!6}
        2B4
        & Transfer Recipient Depending on Transaction Order ~\citeA{vidal2024openscv}
        & \\

        
        2C 
        & Bad random number generation~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-120/}{SWC-120}, \bluelink{https://owasp.org/www-project-smart-contract-top-10/2025/en/src/SC09-insecure-randomness.html}{OWASP-SC09}, \bluelink{https://dasp.co/\#item-6}{DASP-6}, Generating Randomness~\cite{Rameder2022}~\citeA{ ZhouEtAl2022, Staderini2022},
        Bad randomness~\cite{Rameder2022},
        Weak Sources of Randomness from Chain Attributes~\citeA{dZaazaaAndElBakkali2023a,dZaazaaAndElBakkali2023b}, Random Number~\citeA{VivarEtAl2021}, Weak PRNG~\citeA{li2024static}\\

        2C1
        & Randomness Using Block Hash~\citeA{KushwahaEtAl2022a}
        & \\

        \rowcolor{gray!6}        
        2D 
        & Leakage of confidential information~\cite{Rameder2022} 
        & \bluelink{https://swcregistry.io/docs/SWC-136/}{SWC-136}, Lack of transaction privacy~\cite{Rameder2022}~\citeA{ KushwahaEtAl2022a},
        Private information leakage, Nothing is secret, Confidentiality failure, Keeping secrets, Data exposure~\cite{Rameder2022},
        On-chain oracle manipulation~\citeA{ChaliasosEtAl2024}, Secrecy failure~\citeA{Staderini2022}, Exposed secret~\citeA{MunirAndTaha2023}, Unencrypted private data on-chain~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}, Secrets~\citeA{VivarEtAl2021} \\
    
        2E
        & Unpredictable state~\cite{Rameder2022}~\citeA{ VivarEtAl2021}
        & Unsafe External Library Call, External Library Calling~\citeA{vidal2024openscv}\\

        2E1
        & Dynamic Library~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\

        2E2
        & References to destroyed contracts~\citeA{MunirAndTaha2023}
        & \\

        2E3
        & Use of Malicious Libraries~\citeA{vidal2024openscv}
        & Using components with known vulnerabilities~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, External Library Calling, Malicious Libraries~\citeA{vidal2024openscv} \\
        
        2E4
        & External Contract Referencing~\citeA{ZhouEtAl2022}
        & Misuse of address parameters in the constructor~\citeA{MunirAndTaha2023}, Value assigned to contract address~\citeA{DiasEtAl2021}\\

        \rowcolor{gray!6}
        
        2F
        & Unsafe Non-Blockchain External Call~\citeA{vidal2024openscv}
        &  \\
        \rowcolor{gray!6}
        2F1
        & Unsafe External Web Service Call~\citeA{vidal2024openscv}
        & Web Service~\citeA{vidal2024openscv} \\
        \rowcolor{gray!6}
        2F2
        & Unsafe External Command Execution~\citeA{vidal2024openscv}
        & System Command Execution~\citeA{vidal2024openscv} \\
        \rowcolor{gray!6}
        2F3
        & Unsafe External File Access~\citeA{vidal2024openscv}
        & External File Accessing~\citeA{vidal2024openscv} \\
        
        2G
        & Cross Channel Invocation~\citeA{vidal2024openscv}
        & Cross Channel Chaincode Invocation~\citeA{vidal2024openscv} \\
        
        \midrule
        \multicolumn{3}{l}{\textbf{3 - Exception \& Error Handling Disorders}}\\
        \midrule
        \rowcolor{gray!6}
        3A
        & Unchecked low-level call/send return values~\cite{Rameder2022}
        & \bluelink{https://owasp.org/www-project-smart-contract-top-10/2025/en/src/SC06-unchecked-external-calls.html}{OWASP-SC06}, \bluelink{https://dasp.co/\#item-4}{DASP-4}, Unhandled exception, Mishandled exceptions~\cite{Rameder2022}~\citeA{ChuEtAl2023},
        Improper handling of exceptions~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Improper Check of Low-Level Call Return Value~\citeA{vidal2024openscv}, Unchecked external calls~\citeA{ChenEtAl2022}, Check on external call~\citeA{MunirAndTaha2023}, Improper Check of External Call Return Value, Improper Exception Handling of External Calls~\citeA{vidal2024openscv}
        \\
        \rowcolor{gray!6}
        3A1
        & Unchecked call~\citeA{li2024static}
        & \bluelink{https://swcregistry.io/docs/SWC-104/}{SWC-104}, Unchecked call return values~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022, Staderini2022}\\
        \rowcolor{gray!6}
        3A2
        & Unchecked send~\citeA{li2024static}
        & Unchecked/unsafe send~\cite{Rameder2022}\\
        \rowcolor{gray!6}
        3A3
        & Unchecked transfer~\citeA{li2024static}~\cite{slither}
        & Improper Check on Transfer Credit~\citeA{vidal2024openscv}\\

        
        3B
        & Unexpected throw or revert~\cite{Rameder2022}
        &  Improper Use of Exception Handling Functions~\citeA{vidal2024openscv}\\

        3B1
        & Mishandled out-of-gas exception~\cite{Rameder2022}
        & Gasless send\cite{Rameder2022}~\citeA{ Staderini2022, KushwahaEtAl2022a}\\

        \rowcolor{gray!6}
        3C
        & Assert, require or revert violation~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-123/}{SWC-123}, \bluelink{https://swcregistry.io/docs/SWC-110/}{SWC-110}, Assert violation~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Assertion failure~\citeA{ChoiEtAl2021},
        Requirement violation~\citeA{ChoiEtAl2021, WeiEtAl2023, Staderini2022},
        Requirement violation by the called smart contract~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Require on input variable~\citeA{DiasEtAl2021},
        Revert require, Exception state~\citeA{AgarwalEtAl2022}\\
        \rowcolor{gray!6}
        3C1
        & Wrong Selection of Guard Function~\citeA{vidal2024openscv}
        & \\
        
        3D
        & Send instead of transfer
        & Wrong use of transfer credit function~\citeA{vidal2024openscv}\\
        
        \midrule
        \multicolumn{3}{l}{\textbf{4 - Denial of Service}}\\
        \midrule
        \rowcolor{gray!6}
        4A
        & Greedy contract~\cite{Rameder2022}
        & Locked Ether~\cite{Rameder2022},
        Freezing Ether~\citeA{Staderini2022, ZhouEtAl2022, ChoiEtAl2021, KushwahaEtAl2022b}\\
        \rowcolor{gray!6}
        4A1
        & Locked Money~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022, ChuEtAl2023} 
        & Unreachable Payable Function~\citeA{vidal2024openscv}\\
        \rowcolor{gray!6}
        4A2
        & Frozen Ether~\cite{Rameder2022}
        & \\

        4B
        & Ether lost in transfer\cite{Rameder2022} 
        & Transfer to orphan address~\cite{Rameder2022},
        Lost of Ether~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, KushwahaEtAl2022a}, Loss of Ether~\citeA{VivarEtAl2021}\\

        \rowcolor{gray!6}
        4C
        & DoS with block gas limit reached~\cite{Rameder2022}~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, KushwahaEtAl2022a}
        & \bluelink{https://swcregistry.io/docs/SWC-128/}{SWC-128},
        Check on gas Limit~\citeA{DiasEtAl2021},
        Gas limit in loops, Extra Gas in loop~\citeA{AgarwalEtAl2022}, DoS with block gas limit~\citeA{li2024static} \\
        \rowcolor{gray!6}
        % DoS Costly Pattern and Loops~\citeA{Staderini2022} è stato spostato. Prima era nome alternativo di 4C. Ora è rappresentante di 4C1. Il vecchio rappresentante di 4C1 è stato spostato come nome alternativo di 4C1.
        4C1
        & DoS Costly Pattern and Loops~\citeA{Staderini2022}
        & Multiple calls in a single transaction~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Nested Call~\citeA{ChenEtAl2022}, Multiple calls, Transfer in loop~\citeA{AgarwalEtAl2022}\\
        \rowcolor{gray!6}        
        4C2
        & Array length manipulation~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022}
        & Unsafe array length Assignment~\citeA{li2024static}\\
        \rowcolor{gray!6}
        4C3
        & Infinite loop~\citeA{WeiEtAl2023}
        & Unbounded mass operation~\citeA{MunirAndTaha2023} \\
        
        4D
        & DoS by Exception inside loop~\cite{Rameder2022}
        & DoS under external influence~\cite{Rameder2022}~\citeA{ ChenEtAl2022}, Wallet griefing causing out of gas exception~\cite{Rameder2022}, Improper Exception Handling in a Loop~\citeA{vidal2024openscv} \\

        \rowcolor{gray!6}
        4E
        & Insufficient gas griefing~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023, WeiEtAl2023, KushwahaEtAl2022a}
        & \bluelink{https://swcregistry.io/docs/SWC-126/}{SWC-126}, Incorrect Revert Implementation in a Loop~\citeA{vidal2024openscv}\\

        4F
        & Overpowered Role~\citeA{AgarwalEtAl2022}
        & Check on overpowered role~\citeA{DiasEtAl2021} \\

        \rowcolor{gray!6}
        4G
        & Missed to implement a fallback function~\citeA{MunirAndTaha2023}
        & \\

        4H
        & Improper locking during external calls~\citeA{vidal2024openscv}
        & \\

        \rowcolor{gray!6}
        4I
        & DoS with failed call~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023, KushwahaEtAl2022a}
        & \bluelink{https://swcregistry.io/docs/SWC-113/}{SWC-113}, Unexpected-throw-DoS, DoS with unexpected revert/throw\cite{Rameder2022}, Dos by External contracts~\cite{Rameder2022}~\citeA{ Staderini2022}\\
        
        4J
        & Unsafe send() in the require() condition~\citeA{li2024static}
        & \\
        
        \midrule
        \multicolumn{3}{l}{\textbf{5 - Resource Consumption \& Gas Related Issues}}\\
        \midrule
        \rowcolor{gray!6}
        5A 
        & Gas costly loops~\cite{Rameder2022} 
        & Invariants in loops~\cite{Rameder2022} \\

        5B
        & Gas costly pattern~\cite{Rameder2022}
        & Inefficient Operation Sequence~\citeA{vidal2024openscv}\\

        \rowcolor{gray!6}
        5C
        & High gas consumption of variable data type or declaration
        & \\
        \rowcolor{gray!6}
        5C1
        & Byte Array~\cite{Rameder2022}
        & Variable type~\citeA{DiasEtAl2021}, Bytes Variables Risk~\citeA{li2024static}, Wrong Type in Variable Declaration~\citeA{vidal2024openscv}\\
        \rowcolor{gray!6}
        5C2
        & Invariant State variables not declared constant~\cite{Rameder2022} 
        & Declaration of invariant state variable~\citeA{DiasEtAl2021}, Missing Constant Modifier in Variable Declaration~\citeA{vidal2024openscv} \\

        5D
        & High gas consumption function type~\cite{Rameder2022}~\citeA{ ChenEtAl2022}
        & Function declaration public instead of external~\cite{Rameder2022}~\citeA{vidal2024openscv}\\

        \rowcolor{gray!6}
        5E 
        & Under-priced opcodes~\cite{Rameder2022}
        & \\

        5F
        & Transfer of all the gas~\cite{Rameder2022}
        & \\

        \midrule
        \multicolumn{3}{l}{\textbf{6 - Authentication \& Access Control Vulnerabilities}}\\
        \midrule
        \rowcolor{gray!6}
        6A
        & Prodigal contract
        & \\
        \rowcolor{gray!6}
        6A1
        & Authorization via transaction origin~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-115/}{SWC-115}, Authentication through tx.origin~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, Staderini2022, AgarwalEtAl2022, ZhouEtAl2022, KushwahaEtAl2022a},
        Transaction state dependency~\citeA{MunirAndTaha2023, luo2024scvhunter},
        Transaction origin use~\citeA{ChoiEtAl2021}, Dangerous Usage of tx.origin~\citeA{li2024static}, Wrong Caller Identification~\citeA{vidal2024openscv}  \\

        6B
        & Access Control management~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \bluelink{https://owasp.org/www-project-smart-contract-top-10/2025/en/src/SC01-access-control.html}{OWASP-SC01}, \bluelink{https://dasp.co/\#item-2}{DASP-2}, Improper access control~\citeA{vidal2024openscv} \\
        
        6B1
        & Unprotected self-destruction~\cite{Rameder2022}~\citeA{ ChuEtAl2023, AgarwalEtAl2022, KushwahaEtAl2022a, KushwahaEtAl2022b, Staderini2022, ZhouEtAl2022}
        & \bluelink{https://swcregistry.io/docs/SWC-106/}{SWC-106}, Unexpected kill, Destroyable contract~\cite{Rameder2022},
        Suicidal contract~\citeA{ChoiEtAl2021},
        Unsafe suicide~\citeA{WeiEtAl2023},
        Check on suicide functionality~\citeA{DiasEtAl2021}\\

        6B2
        & Unauthorized Ether withdrawal~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-105/}{SWC-105}, Unprotected Ether withdrawal~\citeA{Staderini2022, WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, KushwahaEtAl2022a}
        Check on balance withdrawal~\citeA{DiasEtAl2021},
        Ether leak~\citeA{ChoiEtAl2021} \\

        6B3
        & Initializing method without permission check~\citeA{li2024static}
        &  \\

        6B4
        & Missing msg.sender check for transferFrom()~\citeA{li2024static}
        & Arbitrary from in transferFrom() without msg.sender check~\citeA{li2024static} \\

        6B5
        & Sending Ether to arbitrary destinations~\citeA{li2024static}
        &  \\

        6B6
        & Unauthorized accessibility due to wrong function or state variable visibility~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-108/}{SWC-108}, Visibility of exposed functions~\cite{Rameder2022}~\citeA{ Staderini2022}
        Function or state variable default visibility~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Function/State visibility error~\citeA{ChaliasosEtAl2024},
        Unspecified visibility level~\citeA{MunirAndTaha2023},
        Bad visibility~\citeA{AgarwalEtAl2022},
        Default visibility~\citeA{ZhouEtAl2022},
        No restricted write, Implicit visibility level, Non-public variables accessed by public/external functions, Default/Unintended/Erroneous visibility~\cite{Rameder2022} \\

        6B6.1
        & Function default visibility~\citeA{WeiEtAl2023, KushwahaEtAl2022a}
        & \bluelink{https://swcregistry.io/docs/SWC-100/}{SWC-100}, Default function visibility~\citeA{li2024static}, Wrong function modifier~\citeA{vidal2024openscv}\\

        6B6.2
        & State variable default visibility~\citeA{WeiEtAl2023}
        & Missing visibility modifier in variable declaration~\citeA{vidal2024openscv}\\

        6B7
        & Bypassable Modifier~\citeA{fang2023beyond}
        & \\
        
        \rowcolor{gray!6}
        6C
        & Signature based vulnerabilities~\cite{Rameder2022}
        & Insufficient signature information~\cite{Rameder2022} \\
        \rowcolor{gray!6}
        6C1
        & Missing protection against signature replay attack~\cite{Rameder2022}~\citeA{ Staderini2022, WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \bluelink{https://swcregistry.io/docs/SWC-121/}{SWC-121}, Improper Check against Signature Replay Attacks~\citeA{vidal2024openscv}\\
        \rowcolor{gray!6}
        6C2 
        & Lack of proper signature verification~\cite{Rameder2022}~\citeA{ WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \bluelink{https://swcregistry.io/docs/SWC-122/}{SWC-122}, Method permit() Used for Arbitrary from in transferFrom()~\citeA{li2024static}, Improper authenticity check~\citeA{vidal2024openscv}\\
        \rowcolor{gray!6}
        6C3
        & Hash collision with multiple variable length arguments~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, KushwahaEtAl2022a}
        & \bluelink{https://swcregistry.io/docs/SWC-133/}{SWC-133}, Incorrect Argument Encoding~\citeA{vidal2024openscv}\\
        \rowcolor{gray!6}
        6C4
        & Function Clashing~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\
        \rowcolor{gray!6}
        6C5
        & Signature Malleability~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022, WeiEtAl2023}
        & \bluelink{https://swcregistry.io/docs/SWC-117/}{SWC-117}, Incorrect Verification of Cryptographic Signature~\citeA{vidal2024openscv}\\
        \rowcolor{gray!6}
        6C6
        & Map overlap~\citeA{MunirAndTaha2023}
        & \\

        6D
        & Identity Verification~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\
        \rowcolor{gray!6}
        6E
        & Usage of public mint or burn~\citeA{li2024static}
        & \\
        
        \midrule
        \multicolumn{3}{l}{\textbf{7 - Arithmetic bugs}}\\
        \midrule

        7A
        & Integer over- or underflow~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, Staderini2022, KushwahaEtAl2022a, AgarwalEtAl2022, ChuEtAl2023, MunirAndTaha2023}
        & \bluelink{https://swcregistry.io/docs/SWC-101/}{SWC-101}, \bluelink{https://owasp.org/www-project-smart-contract-top-10/2025/en/src/SC08-integer-overflow-underflow.html}{OWASP-SC08}, \bluelink{https://dasp.co/\#item-3}{DASP-3}, Arithmetic UnderflowOverflow~\citeA{KushwahaEtAl2022b},
        Integer bug~\citeA{ChoiEtAl2021},
        Value assignment with too many digits~\citeA{DiasEtAl2021} \\

        7A1
        & Integer overflow~\citeA{vidal2024openscv}
        &  \\

        7A2
        & Integer underflow~\citeA{vidal2024openscv}
        &  \\

        \rowcolor{gray!6}
        7B
        & Unchecked division~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\
        \rowcolor{gray!6}
        7B1
        & Integer division~\cite{Rameder2022}
        & Money leak~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Unexpected result from division~\citeA{MunirAndTaha2023}, Floating point \& Precision~\cite{Rameder2022} \\
        \rowcolor{gray!6}
        7B2
        & Integer Division before Multiplication~\citeA{li2024static}
        & Arithmetic Precision~\citeA{Staderini2022}\\
        \rowcolor{gray!6}
        7B3
        & Divide by Zero~\citeA{vidal2024openscv}
        & \\

    
        7C
        & Integer bugs or Arithmetic Issues~\cite{Rameder2022}
        & Check on arithmetic operation~\citeA{DiasEtAl2021},
        Unchecked Math, Wrong operator~\cite{Rameder2022}\\

        7C1
        & Incorrect Calculation~\citeA{li2024cobra}
        & \\

        7C2
        & Truncation Bugs~\citeA{AgarwalEtAl2022, vidal2024openscv}
        & Integer Truncation~\cite{Rameder2022}~\citeA{ DiasEtAl2021}\\

        7C3
        & Signedness Bugs~\citeA{AgarwalEtAl2022, vidal2024openscv}
        & Integer sign~\cite{Rameder2022}~\citeA{ DiasEtAl2021}\\

        \midrule
        \multicolumn{3}{l}{\textbf{8 - Bad Coding Quality and Programming Language Specifics}}\\
        \midrule
        \rowcolor{gray!6}
        8A
        & Type cast~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, Staderini2022}
        & Unsafe type declaration, Type conversion~\citeA{VivarEtAl2021}, Wrong Function Call~\citeA{vidal2024openscv} \\

        8B
        & Coding error~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-129/}{SWC-129}, Typographical error~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, vidal2024openscv}, Immutable bugs~\cite{Rameder2022}~\citeA{ VivarEtAl2021}, Coding Bug\cite{Rameder2022} \\

        \rowcolor{gray!6}
        8C
        & Bad coding pattern~\cite{Rameder2022}
        & \\

        8D
        & Deprecated source language features~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-111/}{SWC-111}, Use of deprecated Solidity function~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} \\

        % 8E
        % & Write to arbitrary storage location~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, DiasEtAl2021}
        % & Arbitrary send~\citeA{AgarwalEtAl2022},
        % Arbitrary write~\citeA{ChoiEtAl2021} \\

        \rowcolor{gray!6}
        8E
        & Use of assembly~\cite{Rameder2022}~\citeA{ AgarwalEtAl2022}
        & Assembly-based vulnerabilities~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Usage of assembly~\citeA{AgarwalEtAl2022}\\
        \rowcolor{gray!6}
        8E1
        & Arbitrary jump with function type variable~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}
        & \bluelink{https://swcregistry.io/docs/SWC-127/}{SWC-127}, Arbitrary jump~\citeA{Staderini2022}, Control-Flow hijack~\citeA{ChoiEtAl2021}, Function type variables assignment using arbitrary values~\citeA{DiasEtAl2021}, Specify function variable as any type\cite{Rameder2022} \\
        \rowcolor{gray!6}
        8E2
        & Constant function using assembly code~\citeA{AgarwalEtAl2022} 
        & Constant Function~\citeA{AgarwalEtAl2022}, Interoperability issues with other contracts~\citeA{vidal2024openscv} \\
        \rowcolor{gray!6}
        8E3
        & Returning results using assembly code in constructor~\cite{Rameder2022}
        & \\
        
        8F
        & Incorrect inheritance order~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}
        & \bluelink{https://swcregistry.io/docs/SWC-125/}{SWC-125}, Wrong class inheritance order~\citeA{vidal2024openscv}\\

        \rowcolor{gray!6}
        8G
        & Variable shadowing~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-119/}{SWC-119}, Hidden state variable~\cite{Rameder2022},
        Shadowing state variables~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Variable name~\citeA{DiasEtAl2021},
        Tained memory~\citeA{MunirAndTaha2023},
        Shadowing state, Shadowing abstract, Shadowing builtin, Shadowing local~\citeA{AgarwalEtAl2022} \\
        \rowcolor{gray!6}
        8G1
        & Use of Same Variable or Function Name In Inherited Contract~\citeA{vidal2024openscv}
        &  \\
        \rowcolor{gray!6}
        8G2
        & Variables or Functions Named After Reserved Words~\citeA{vidal2024openscv}
        &  \\
        \rowcolor{gray!6}
        8G3
        & Use of the Same Variable or Function Name In a Single Contract~\citeA{vidal2024openscv}
        &  \\
        

        8H 
        & Misleading source code~\cite{Rameder2022}
        & API inconsistency~\cite{Rameder2022} \\

        8H1
        & Right to Left override~\citeA{Staderini2022, WeiEtAl2023}~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-130/}{SWC-130}, Function Call with Wrong Arguments~\citeA{vidal2024openscv}\\

        8H2
        & Misleading data location~\citeA{ChenEtAl2022}
        & Modifying storage array by value~\citeA{li2024static}\\

        8H3
        & Hidden built-in symbols~\cite{Rameder2022}
        & Built-in symbol shadowing~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b},
        Use of deprecated built-in symbols~\citeA{DiasEtAl2021} \\

        \rowcolor{gray!6}
        8I
        & Missing logic~\cite{Rameder2022} 
        & \bluelink{https://owasp.org/www-project-smart-contract-top-10/2025/en/src/SC03-logic-errors.html}{OWASP-SC03}, Logical errors or dead code~\cite{Rameder2022}, Business logic vulnerabilities, Wrong logic~\citeA{vidal2024openscv}\\
        \rowcolor{gray!6}
        8I1
        & Code with no effects~\cite{Rameder2022}~\citeA{ WeiEtAl2023, dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} 
        & \bluelink{https://swcregistry.io/docs/SWC-135/}{SWC-135}, No Effect Code Execution~\citeA{vidal2024openscv}\\
        \rowcolor{gray!6}
        8I2
        & Unused variable~\citeA{vidal2024openscv} 
        & \bluelink{https://swcregistry.io/docs/SWC-131/}{SWC-131}, Presence of unused variables~\cite{Rameder2022}~\citeA{ WeiEtAl2023}\\
        \rowcolor{gray!6}
        8I3
        & Unused return~\citeA{AgarwalEtAl2022, li2024static}
        & ~\\
        \rowcolor{gray!6}
        8I4
        & Unused statement~\citeA{ChenEtAl2022}
        & \\
        \rowcolor{gray!6}
        8I5
        & Missing return type on function~\citeA{vidal2024openscv}
        & \\
        \rowcolor{gray!6}
        8I6
        & Missing type in variable declaration~\citeA{vidal2024openscv}
        & Insecure inference~\citeA{MunirAndTaha2023},
        Unsafe type inference~\cite{Rameder2022}\\
        \rowcolor{gray!6}
        8I7
        & Missing variable initialization~\citeA{vidal2024openscv}
        & Uninitialized local/state variable~\cite{Rameder2022},
        Uninitialized state variables~\citeA{ChuEtAl2023},
        Uninitialized state, Uninitialized local~\citeA{AgarwalEtAl2022},
        Initialization of local variables, Initialization of state variables, Missing initialization~\citeA{DiasEtAl2021}\\
        \rowcolor{gray!6}
        8I8
        & Missing input validation~\citeA{li2024static}
        & \bluelink{https://owasp.org/www-project-smart-contract-top-10/2025/en/src/SC04-lack-of-input-validation.html}{OWASP-SC04}, Improper input validation~\citeA{vidal2024openscv}\\
        \rowcolor{gray!6}
        8I9
        & Function return type mismatch~\citeA{vidal2024openscv}
        & \\
        \rowcolor{gray!6}
        8I10
        & Parameter type mismatch~\citeA{vidal2024openscv}
        & \\
        \rowcolor{gray!6}
        8I11
        & Wrong type of Function~\citeA{vidal2024openscv}
        & \\
        \rowcolor{gray!6}
        8I12
        & Redundant Functionality~\citeA{vidal2024openscv}
        & \\


        8J
        & Insecure contract upgrading~\cite{Rameder2022}
        & Upgradable contract, Patching~\cite{Rameder2022} \\

        \rowcolor{gray!6}
        8K
        & Inadequate or incorrect logging or documentation~\cite {Rameder2022}
        & \\

        8L
        & Hardcoded addresses~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022, ChenEtAl2022, vidal2024openscv}
        & \\

        \rowcolor{gray!6}

        8M
        & Send to zero address~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\


        8N
        & Double constructor~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & \\
                    
        \rowcolor{gray!6}
        8O
        & Missing constructor~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, vidal2024openscv}
        & \\

        8P
        & Extraneous Field Declaration~\citeA{vidal2024openscv}
        & \\
        
        \rowcolor{gray!6}
        8Q
        & Inadequate Data Representation~\citeA{vidal2024openscv}
        & \\

        \midrule
        \multicolumn{3}{l}{\textbf{9 - Environment Configuration Issues}}\\
        \midrule

        9A
        & Short address~\cite{Rameder2022}~\citeA{ ZhouEtAl2022, ChuEtAl2023, Staderini2022}
        & \bluelink{https://dasp.co/\#item-9}{DASP-9}, Check on input address length~\citeA{DiasEtAl2021},
        Address shortening~\citeA{MunirAndTaha2023} \\

        \rowcolor{gray!6}        
        9B
        & Outdated compiler version~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023, vidal2024openscv}
        & \bluelink{https://swcregistry.io/docs/SWC-102/}{SWC-102}, Pragmas version~\citeA{AgarwalEtAl2022},
        Unspecified Compiler version~\citeA{ChenEtAl2022},
        Compiler version~\citeA{DiasEtAl2021} \\

        9C
        & Floating or no pragma~\cite{Rameder2022}~\citeA{ WeiEtAl2023, KushwahaEtAl2022a}
        & \bluelink{https://swcregistry.io/docs/SWC-103/}{SWC-103}, Floating compiler version~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Undetermined program version prevalence~\citeA{vidal2024openscv} \\

        \rowcolor{gray!6}
        9D
        & Token API violation~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Token standard incompatibility~\cite{Rameder2022}, Unmatched ERC-20 Standard~\citeA{ChenEtAl2022}, Extraneous exception handling~\citeA{vidal2024openscv} \\
        \rowcolor{gray!6}
        9D1
        & Improper or missing event handling~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}
        & Missing Reminder~\citeA{ChenEtAl2022}, Fake Deposit~\citeA{MunirAndTaha2023}, Missing token verification of exchange~\citeA{vidal2024openscv} \\
        \rowcolor{gray!6}
        9D2
        & ERC-20 transfer~\citeA{vidal2024openscv}
        & \\
        

        9E
        & Ethereum update incompatibility~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-134/}{SWC-134}, Failing to accept new deposit, Deposit Acceptance~\citeA{MunirAndTaha2023},
        Message call with hardcoded gas amount~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023}\\

        9E1
        & Call with hardcoded gas amount~\citeA{vidal2024openscv}
        & \\

        9E2
        & transfer() and send() with hardcoded gas amount~\citeA{vidal2024openscv}
        & \\
        
        \rowcolor{gray!6}
        9F
        & Configuration error~\cite{Rameder2022}
        & \\

        9G
        & Missing Interrupter~\citeA{ChenEtAl2022}
        & \\

        \midrule
        \multicolumn{3}{l}{\textbf{10 - Eliminated/Deprecated syntax}}\\
        \midrule
        
        \rowcolor{gray!6}
        10A
        & Callstack depth limit~\cite{Rameder2022}
        & Stack size limit~\cite{Rameder2022}, 
        Limited stack size~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Stack size~\citeA{VivarEtAl2021} \\

        10B
        & Uninitialized storage pointer~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, MunirAndTaha2023, vidal2024openscv}
        & \bluelink{https://swcregistry.io/docs/SWC-109/}{SWC-109}, Uninitialized storage~\citeA{AgarwalEtAl2022}, Initialization of storage pointer~\citeA{DiasEtAl2021} \\

        \rowcolor{gray!6}
        10C
        & Erroneous constructor name~\cite{Rameder2022}
        & \bluelink{https://swcregistry.io/docs/SWC-118/}{SWC-118}, Incorrect constructor name~\cite{Rameder2022}~\citeA{ dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, WeiEtAl2023},
        Constructor name~\citeA{DiasEtAl2021}, Wrong constructor name~\citeA{vidal2024openscv}\\

        10D
        & Deprecated APIs~\citeA{ChenEtAl2022}
        & \\

        \midrule
        \multicolumn{3}{l}{\textbf{11 - Library Misuses}}\\
        \midrule
        \rowcolor{gray!6}
        11A & Invalid Wrapper Check in Library~\citeA{Huang2024Revealing} & \\

        11B & Unhandled Exceptions in Library~\citeA{Huang2024Revealing} & \\
        \rowcolor{gray!6}
        11C & Inappropriate Library Extension~\citeA{Huang2024Revealing} & \\

        11D & Inappropriate Using For~\citeA{Huang2024Revealing} & \\
        \rowcolor{gray!6}
        11E & Incomplete Function Replacement~\citeA{Huang2024Revealing} & \\

        11F & Overestimated Library Capability~\citeA{Huang2024Revealing} & \\
        \rowcolor{gray!6}
        11G & Underestimated Library Capability~\citeA{Huang2024Revealing} & \\

        11H & Unnecessary Library Using~\citeA{Huang2024Revealing} & \\

        \midrule
        \multicolumn{3}{l}{\textbf{12 - Machine Unauditable Functional Vulnerabilities}}\\
        \midrule
        
        \rowcolor{gray!6}
        12A & Price oracle manipulation~\citeA{sun2024gptscan} & \bluelink{https://owasp.org/www-project-smart-contract-top-10/2025/en/src/SC02-price-oracle-manipulation.html}{OWASP-SC02}, Price manipulation~\citeA{sun2024gptscan, wang2024skyeye}\\
        \rowcolor{gray!6}
        12A1 & Price oracle manipulation with AMM~\citeA{sun2024gptscan} & \\
        \rowcolor{gray!6}
        12A2 & Price oracle manipulation by buying token~\citeA{sun2024gptscan} & \\

        12B & Erroneous Accounting~\citeA{Z.ZhangEtAl2023} & \\
        
        \rowcolor{gray!6}
        12C & ID Uniqueness Violation~\citeA{wang2024smartinv} & ID-related violation~\citeA{Z.ZhangEtAl2023}\\

        12D & Inconsistent State Updates~\citeA{wang2024smartinv} & Erroneous State Updates~\citeA{Z.ZhangEtAl2023}\\

        \rowcolor{gray!6}
        12E & Privilege Escalation~\citeA{Z.ZhangEtAl2023, wang2024smartinv} & \\

        12F & Atomicity Violation~\citeA{Z.ZhangEtAl2023, wang2024smartinv} & \\

        \rowcolor{gray!6}
        12G & Contracts Implementation Specific Bugs~\citeA{Z.ZhangEtAl2023} & \\

        12H & Business Logic Flaw~\citeA{wang2024smartinv} & \\

        \rowcolor{gray!6}
        12I & Cross-Bridge~\citeA{wang2024smartinv} & \\

        \midrule
        \multicolumn{3}{l}{\textbf{13 - Storage \& Memory}}\\
        \midrule
        
        13A & Memory Manipulation~\citeA{li2024static} & \\
        13A1 & Write to arbitrary storage location~\citeA{vidal2024openscv, Rameder2022} & \bluelink{https://swcregistry.io/docs/SWC-124/}{SWC-124}, Arbitrary write~\citeA{ChoiEtAl2021}\\
        13A2 & Read from Arbitrary Storage Location~\citeA{vidal2024openscv} & \\

        \rowcolor{gray!6}
        13B & Static array out-of-bounds~\citeA{song2022esbmc} & \\

        13C & Dynamic array out-of-bounds~\citeA{song2022esbmc} & \\

        \rowcolor{gray!6}
        13D & Dangerous usage of msg.value inside a Loop & \\

        \midrule
        \multicolumn{3}{l}{\textbf{14 - Cross-chain System Vulnerabilities}}\\
        \midrule
        
        14A & Block expansion attack~\cite{kaur2020scalability}\cite{duan2023attacks} & \\
        
        \rowcolor{gray!6}
        14B & Data synchronization timeout attack~\cite{suhail2022blockchain} \cite{duan2023attacks} & \\

        14C & Failure diffusion~\cite{yu2019challenge} \cite{duan2023attacks} & \\

        \rowcolor{gray!6}
        14D & Privacy leakage attack~\cite{xu2022banks} \cite{duan2023attacks} & \\

        14E & Unauthorized access~\cite{rizvi2020identifying} \cite{duan2023attacks} & \\

        \rowcolor{gray!6}
        14F & Disguised and untrusted notary~\cite{sun2020collaborative} \cite{duan2023attacks} & \\

        14G & Transaction forgery attack~\cite{lv2022attack} \cite{duan2023attacks} & \\

        \rowcolor{gray!6}
        14H & Denial of service attack~\cite{tian2021enabling} \cite{duan2023attacks} & \\

        14I & Hot wallet attack~\cite{chepurnoy2019multi} \cite{duan2023attacks} & \\

        \rowcolor{gray!6}
        14J & Wormhole attack~\cite{malavolta2018anonymous} \cite{duan2023attacks} & \\

        14K & Sore loser attack~\cite{xue2021hedging} \cite{duan2023attacks} & \\

        \rowcolor{gray!6}
        14L & Routing attack~\cite{careem2020reputation} \cite{duan2023attacks} & \\

        14M & Replay attack~\cite{sonnino2020replay} \cite{duan2023attacks} & \\

        \rowcolor{gray!6}
        14N & Collusion attack~\cite{schrepel2019collusion} \cite{duan2023attacks} & \\

        14O & Unrestricted Deposit Emitting~\cite{zhang2022xscope} \cite{duan2023attacks} & \\

        \rowcolor{gray!6}
        14P & Inconsistent Event Parsing~\cite{zhang2022xscope} \cite{duan2023attacks} & \\

        14Q & Unauthorized Unlocking~\cite{zhang2022xscope} \cite{duan2023attacks} & \\

\end{longtable}
}

==> tables/to_validate.tex <==
{
\tiny
\begin{longtable}{p{0.5cm} p{7.2cm} p{7.3cm}}
    \caption{A Comprehensive List of Vulnerabilities Hierarchically Organized.}
    \label{tab:final_tax}\\
    \toprule
    \textbf{Id} & \textbf{Name} & \textbf{Alternative Names} \\
    \midrule
    \endfirsthead
    \multicolumn{3}{c}{{Continued from previous page}} \\
    \toprule
    \textbf{Id} & \textbf{Name} & \textbf{Alternative Names} \\ 
    \midrule
    \endhead
    \midrule
    \multicolumn{3}{r}{{Continued on next page}} \\
    \midrule
    \endfoot
    \bottomrule
    \endlastfoot

    \multicolumn{3}{l}{\textbf{1 - Malicious Environment, Transactions, or Input}}\\
    \midrule
    
        
       
        
       
        1A1.3 & Reentrancy with same effect~\citeA{li2024static} & Reentrancy benign~\citeA{AgarwalEtAl2022}~\cite{slither}\\
        1A1.4 & Reentrancy with negative events~\citeA{li2024static} & Reentrancy events~\citeA{AgarwalEtAl2022}~\cite{slither}\\
        
       
        \midrule
        \multicolumn{3}{l}{\textbf{2 - Blockchain/Environment Dependency}}\\
        \midrule

        2A & Block State Dependency~\citeA{ChenEtAl2022, ChoiEtAl2021} & Block Info Dependency~\citeA{ChenEtAl2022}\\

        2C1 & Randomness Using Block Hash~\citeA{KushwahaEtAl2022a} & \\

        2E1 & Dynamic Library~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} & \\

        2E2 & References to destroyed contracts~\citeA{MunirAndTaha2023} & \\

        2E4 & External Contract Referencing~\citeA{ZhouEtAl2022} & Misuse of address parameters in the constructor~\citeA{MunirAndTaha2023}, Value assigned to contract address~\citeA{DiasEtAl2021}\\        
       
        \midrule
        \multicolumn{3}{l}{\textbf{3 - Exception \& Error Handling Disorders}}\\
        \midrule
        \multicolumn{3}{l}{\textbf{4 - Denial of Service}}\\
        \midrule
        
       
        
        % DoS Costly Pattern and Loops~\citeA{Staderini2022} è stato spostato. Prima era nome alternativo di 4C. Ora è rappresentante di 4C1. Il vecchio rappresentante di 4C1 è stato spostato come nome alternativo di 4C1.
        4C1 & DoS Costly Pattern and Loops~\citeA{Staderini2022} & Multiple calls in a single transaction~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b}, Nested Call~\citeA{ChenEtAl2022}, Multiple calls, Transfer in loop~\citeA{AgarwalEtAl2022}\\
                
        4C2 & Array length manipulation~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b, AgarwalEtAl2022}
        & Unsafe array length Assignment~\citeA{li2024static}\\
        
        4C3 & Infinite loop~\citeA{WeiEtAl2023}
        & Unbounded mass operation~\citeA{MunirAndTaha2023} \\
        
        4F & Overpowered Role~\citeA{AgarwalEtAl2022} & Check on overpowered role~\citeA{DiasEtAl2021} \\

        
        4G & Missed to implement a fallback function~\citeA{MunirAndTaha2023} & \\
        
        4J & Unsafe send() in the require() condition~\citeA{li2024static} & \\
        
        \midrule
        \multicolumn{3}{l}{\textbf{5 - Resource Consumption \& Gas Related Issues}}\\
        \midrule
        
        5C & High gas consumption of variable data type or declaration & \\
        
        \midrule
        \multicolumn{3}{l}{\textbf{6 - Authentication \& Access Control Vulnerabilities}}\\
        \midrule
        
        6A & Prodigal contract & \\
        
       
        
      
      
        6B3 & Initializing method without permission check~\citeA{li2024static} &  \\

        6B4 & Missing msg.sender check for transferFrom()~\citeA{li2024static} & Arbitrary from in transferFrom() without msg.sender check~\citeA{li2024static} \\

        6B5 & Sending Ether to arbitrary destinations~\citeA{li2024static} &  \\

        6B7 & Bypassable Modifier~\citeA{fang2023beyond} & \\

        6C6 & Map overlap~\citeA{MunirAndTaha2023} & \\

        6D & Identity Verification~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} & \\
        
        6E & Usage of public mint or burn~\citeA{li2024static} & \\
        
        \midrule
        \multicolumn{3}{l}{\textbf{7 - Arithmetic bugs}}\\
        \midrule

        
        7B & Unchecked division~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} & \\
       
        7B2 & Integer Division before Multiplication~\citeA{li2024static} & Arithmetic Precision~\citeA{Staderini2022}\\
        
      
        7C1 & Incorrect Calculation~\citeA{li2024cobra} & \\

     
        \midrule
        \multicolumn{3}{l}{\textbf{8 - Bad Coding Quality and Programming Language Specifics}}\\
        \midrule


        8H2 & Misleading data location~\citeA{ChenEtAl2022} & Modifying storage array by value~\citeA{li2024static}\\

       
        8I3 & Unused return~\citeA{AgarwalEtAl2022, li2024static}
        & ~\\
        
        8I4 & Unused statement~\citeA{ChenEtAl2022} & \\
      
        8M & Send to zero address~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} & \\


        8N & Double constructor~\citeA{dZaazaaAndElBakkali2023a, dZaazaaAndElBakkali2023b} & \\
                    
        
        \midrule
        \multicolumn{3}{l}{\textbf{9 - Environment Configuration Issues}}\\
        \midrule

        9G & Missing Interrupter~\citeA{ChenEtAl2022} & \\

        \midrule
        \multicolumn{3}{l}{\textbf{10 - Eliminated/Deprecated syntax}}\\
        \midrule
        
        10D & Deprecated APIs~\citeA{ChenEtAl2022} & \\

        \midrule
        \multicolumn{3}{l}{\textbf{11 - Library Misuses}}\\
        \midrule
        
        11A & Invalid Wrapper Check in Library~\citeA{Huang2024Revealing} & \\

        11B & Unhandled Exceptions in Library~\citeA{Huang2024Revealing} & \\
        
        11C & Inappropriate Library Extension~\citeA{Huang2024Revealing} & \\

        11D & Inappropriate Using For~\citeA{Huang2024Revealing} & \\
        
        11E & Incomplete Function Replacement~\citeA{Huang2024Revealing} & \\

        11F & Overestimated Library Capability~\citeA{Huang2024Revealing} & \\
        
        11G & Underestimated Library Capability~\citeA{Huang2024Revealing} & \\

        11H & Unnecessary Library Using~\citeA{Huang2024Revealing} & \\

        \midrule
        \multicolumn{3}{l}{\textbf{12 - Machine Unauditable Functional Vulnerabilities}}\\
        \midrule
        
        
        12A & Price oracle manipulation~\citeA{sun2024gptscan} & \bluelink{https://owasp.org/www-project-smart-contract-top-10/2025/en/src/SC02-price-oracle-manipulation.html}{OWASP-SC02}, Price manipulation~\citeA{sun2024gptscan, wang2024skyeye}\\
        
        12A1 & Price oracle manipulation with AMM~\citeA{sun2024gptscan} & \\
        
        12A2 & Price oracle manipulation by buying token~\citeA{sun2024gptscan} & \\

        12B & Erroneous Accounting~\citeA{Z.ZhangEtAl2023} & \\
        
        
        12C & ID Uniqueness Violation~\citeA{wang2024smartinv} & ID-related violation~\citeA{Z.ZhangEtAl2023}\\

        12D & Inconsistent State Updates~\citeA{wang2024smartinv} & Erroneous State Updates~\citeA{Z.ZhangEtAl2023}\\

        
        12E & Privilege Escalation~\citeA{Z.ZhangEtAl2023, wang2024smartinv} & \\

        12F & Atomicity Violation~\citeA{Z.ZhangEtAl2023, wang2024smartinv} & \\

        
        12G & Contracts Implementation Specific Bugs~\citeA{Z.ZhangEtAl2023} & \\

        12H & Business Logic Flaw~\citeA{wang2024smartinv} & \\

        
        12I & Cross-Bridge~\citeA{wang2024smartinv} & \\

        \midrule
        \multicolumn{3}{l}{\textbf{13 - Storage \& Memory}}\\
        \midrule
        
        13A & Memory Manipulation~\citeA{li2024static} & \\
       
        13B & Static array out-of-bounds~\citeA{song2022esbmc} & \\

        13C & Dynamic array out-of-bounds~\citeA{song2022esbmc} & \\
 
        13D & Dangerous usage of msg.value inside a Loop & \\

        \midrule
        \multicolumn{3}{l}{\textbf{14 - Cross-chain System Vulnerabilities}}\\
        \midrule
        
        14A & Block expansion attack~\cite{kaur2020scalability}\cite{duan2023attacks} & \\
        
        
        14B & Data synchronization timeout attack~\cite{suhail2022blockchain} \cite{duan2023attacks} & \\

        14C & Failure diffusion~\cite{yu2019challenge} \cite{duan2023attacks} & \\

        
        14D & Privacy leakage attack~\cite{xu2022banks} \cite{duan2023attacks} & \\

        14E & Unauthorized access~\cite{rizvi2020identifying} \cite{duan2023attacks} & \\

        
        14F & Disguised and untrusted notary~\cite{sun2020collaborative} \cite{duan2023attacks} & \\

        14G & Transaction forgery attack~\cite{lv2022attack} \cite{duan2023attacks} & \\

        
        14H & Denial of service attack~\cite{tian2021enabling} \cite{duan2023attacks} & \\

        14I & Hot wallet attack~\cite{chepurnoy2019multi} \cite{duan2023attacks} & \\

        
        14J & Wormhole attack~\cite{malavolta2018anonymous} \cite{duan2023attacks} & \\

        14K & Sore loser attack~\cite{xue2021hedging} \cite{duan2023attacks} & \\
        
        
        14L & Routing attack~\cite{careem2020reputation} \cite{duan2023attacks} & \\

        14M & Replay attack~\cite{sonnino2020replay} \cite{duan2023attacks} & \\

        
        14N & Collusion attack~\cite{schrepel2019collusion} \cite{duan2023attacks} & \\

        14O & Unrestricted Deposit Emitting~\cite{zhang2022xscope} \cite{duan2023attacks} & \\

        
        14P & Inconsistent Event Parsing~\cite{zhang2022xscope} \cite{duan2023attacks} & \\

        14Q & Unauthorized Unlocking~\cite{zhang2022xscope} \cite{duan2023attacks} & \\

\end{longtable}
}

==> tables/tools.tex <==
{
\scriptsize
\begin{longtable}{p{4cm} p{0.6cm} p{0.4cm} p{1.1cm} p{2cm} p{1.2cm} p{1.4cm} p{0.9cm} p{1cm} }
    
    \caption{A Comprehensive List of Tools.}
    \label{tab:tools}\\
    \toprule
    \textbf{Tool} & \textbf{Article} & \textbf{Link} & \textbf{Pub. Date} & \textbf{Language} & \textbf{Bytecode} & \textbf{Source Code} & \textbf{Static} & \textbf{Dynamic} \\ 
    \midrule
    \endfirsthead
    \midrule
    \multicolumn{9}{l}{{Continued from previous page}} \\
    \toprule
    \textbf{Tool} & \textbf{Article} & \textbf{Link} & \textbf{Pub. Date} & \textbf{Language} & \textbf{Bytecode} & \textbf{Source Code} & \textbf{Static} & \textbf{Dynamic} \\ 
    \midrule
    \endhead
    \midrule
    \multicolumn{9}{r}{{Continued on next page}} \\
    \midrule
    \endfoot
    \bottomrule
    \endlastfoot

        SCStudio & \citeA{MengRenEtAl2021} & \href{https://github.com/FISCO-BCOS/SCStudio}{url} & 2021-03 & Python & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        SmartScan & \citeA{SunEtAl2023} & \href{https://smartscan.cs.ryerson.ca:4638/}{url} & 2021-05 & ~ & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        SGUARD & \citeA{MiEtAl2021} & \href{https://github.com/reentrancy/sGuard}{url} & 2021-04 & Node.js & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\ 
        WANA & \citeA{ZhouEtAl2021} & \href{https://github.com/gongbell/wana}{url} & 2020-08 & Python & \ding{51} & ~ & \ding{51} & \ding{51} \\ 
        Artemis & \citeB{WangEtAl2020Artemis} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        SCScan & \citeB{9343119} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        GasFuzzer & \citeB{AshrafEtAl2020} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & \ding{51} \\ 
        DEPOSafe & \citeB{9376204} & ~ & ~ & ~ & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\ 
        ReDefender & \citeA{TorresEtAl2021} & ~ & ~ & ~ & \ding{51} & ~ & ~ & \ding{51} \\ 
        Sooyeon \etal Tool & \citeB{9425913} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        OYENTE (Enanched version) & \citeB{8935603} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        YuXing \etal tool & \citeB{9730357} & ~ & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} \\ 
        Targy (built on sFuzz) & \citeB{9724805} & ~ & ~ & ~ & \ding{51} & ~ & ~ & \ding{51} \\ 
        OYENTE (Enanched version) & \citeB{8870156} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        Pouyan \etal & \citeB{8949045} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        EtherSolve & \citeA{FengEtAl2023} & \href{https://github.com/SeUniVr/EtherSolve/}{url} & 2021-03 & Java & \ding{51} & ~ & \ding{51} & ~ \\ 
        CORREAS \etal (Extends GASOL) & \citeB{3057565} & ~ & ~ & ~ & \ding{51} & \ding{51} & \ding{51} & ~ \\ 
        DeeSCVHunter & \citeA{ControEtAl2021} & \href{https://github.com/MRdoulestar/DeeSCVHunter}{url} & 2021-04 & C & ~ & \ding{51} & \ding{51} & ~ \\ 
        Fuchen et al.  (reinforced FISCO-BCOS-evm) & ~ & \href{https://github.com/FISCO-BCOS/FISCO-BCOS}{url} & 2018-03 & C++ & \ding{51} & ~ & ~ & \ding{51} \\
        Eth2Vec & \citeA{GongEtAl2023} & \href{https://github.com/fseclab-osaka/eth2vec}{url} & 2021-03 & Javascipt, Java & \ding{51} & ~ & \ding{51} & ~ \\ 
        VSCL & \citeA{LinoyEtAl2022} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        ESAF & \citeA{L.ZhangEtAl2022} & \href{https://github.com/alopezvivar/ESAF-PSEUDOCODE}{url} & 2020-11 & Pseudocode & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\ 
        Yuhang \etal & \citeB{Sun_2021} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        Peculiar & \citeA{WuHEtAl2021} & \href{https://github.com/wuhongjun15/Peculiar}{url} & 2021-07 & C & ~ & \ding{51} & \ding{51} & ~ \\ 
        Ben \etal & \citeB{Wang2021SmartCV} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        Wanqing \etal & \citeB{9680540} & ~ & ~ & ~ & \ding{51} & \ding{51} & \ding{51} & ~ \\ 
        EtherProv & \citeA{CaoEtAl2023a} & \href{https://github.com/shomzy/EtherProv}{url} & 2021-10 & Python & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        SmartGift & \citeA{NguyenEtAl2021} & \href{https://github.com/chaoweilanmaohahaha/SmartGift}{url} & 2021-10 & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        AME (CGE) & \citeA{SamreenAndAlalfi2021} & \href{https://github.com/Messi-Q/AMEVulDetector}{url} & 2021-05 & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        SC-VDM & \citeB{SC-VDM} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        Xu \etal & \citeA{ZhukovAndKorkhov2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        GPSCVulDetector & \citeA{ChenEtAl2021} & \href{https://github.com/Messi-Q/GPSCVulDetector}{url} & ~ & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        Jianjun \etal & \citeB{JianjunEtAl2021} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        Ziyuan \etal & \citeB{3444370} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        Shasha \etal & \citeB{101007} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        ReJection & \citeB{e3714a3b32d246f0b781dd55b7d6eec7} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        MENGLIN \etal (Extends Mythril) & \citeB{8867880} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & \ding{51} \\ 
        Yuqi \etal & \citeB{101007978} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        Yang \etal & \citeB{9202747} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        EVMFuzzer & \citeA{JieEtAl2023} & \href{https://github.com/EVMFuzzer/EVMFuzzer}{url} & 2019-08 & Python & \ding{51} & ~ & ~ & \ding{51} \\ 
        CodeNet & \citeA{ChoiEtAl2021} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        EVMPATCH & \citeB{Rodler2020EVMPatchTA} & \href{https://github.com/uni-due-syssec/evmpatch-developer-study}{url} & 2021-08 & Python & \ding{51} & ~ & \ding{51} & \ding{51} \\ 
        SmartConDetect & \citeA{JiangEtAl2021} & \href{https://github.com/s00ne/SmartConDetect}{url} & 2023-09 & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        XFuzz & \citeA{XueEtAl2022} & \href{https://github.com/ToolmanInside/xfuzz_tool }{url} & 2022-06 & C++ & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        RLF & \citeA{JianzhongSuEtAl2022} & \href{https://github.com/Demonhero0/rlf}{url} & 2022-10 & Python & ~ & \ding{51} & ~ & \ding{51} \\ 
        IR-Fuzz & \citeA{AliEtAl2021} & \href{https://github.com/Messi-Q/IR-Fuzz}{url} & 2023-01 & C++ & ~ & \ding{51} & ~ & \ding{51} \\ 
        Ity-Fuzz & \citeA{ShouEtAl2023} & \href{https://github.com/fuzzland/ityfuzz}{url} & 2023-06 & Rust & ~ & \ding{51} & ~ & \ding{51} \\ 
        SafeSmartContracts & \citeB{181106632} & \href{https://github.com/wesleyjtann/Safe-SmartContracts}{url} & 2019-12 & Python & \ding{51} & ~ & \ding{51} & ~ \\ 
        ReChecker (VulDeeSmartContract) & \citeB{8970384} & \href{https://github.com/Messi-Q/ReChecker}{url} & 2020-01 & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        DL-MDF & \citeB{s23167246} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        HCC & \citeB{giesen2022} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        DeFinary (built on SCRepair)  & \citeB{3551349} & \href{https://sites.google.com/view/ase2022-definery}{url} & 2022-08 &  JavaScript & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        JiEtAl2023 & \citeA{JiEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        SmartFast & \citeA{HwangEtAl2022} & \href{https://github.com/SmartContractTools/SmartFast/tree/main}{url} & 2022-10 & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        MSmart & \citeA{HuangEtAl2022} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        SuMo & \citeA{PraitheeshanEtAl2021} & \href{https://github.com/MorenaBarboni/SuMo-SOlidity-Mutator}{url} & 2022-06 & JavaScript & ~ & \ding{51} & ~ & \ding{51} \\ 
        ReSuMo & \citeA{RutaoYuEtAl2021} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        Huang \etal & \citeA{HuEtAl2023a} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        M-A-R & \citeA{L.YuEtAl2023} & \href{https://github.com/woods1060/M-A-R}{url} & 2021-08 & Python & ~ & \ding{51} & ~ & \ding{51} \\ 
        SMARTEST & \citeA{SunbeomSoEtAl2021} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        Porosity & \citeB{suiche2017porosity} & \href{https://github.com/msuiche/porosity}{url} & 2017-01 & C++ & \ding{51} & ~ & \ding{51} & \ding{51} \\ 
        MANDO-GURU & \citeA{LiaoEtAl2022} & \href{https://github.com/MANDO-Project/ge-sc-machine}{url} & 2022-11 & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        MANDO-HGT & \citeA{R.YuEtAl2023} & \href{https://github.com/MANDO-Project/ge-sc-transformer}{url} & 2023-01 & Python & \ding{51} & \ding{51} & \ding{51} & ~ \\ 
        SCGRU & \citeA{DuanEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        VulHunter & \citeA{QianEtAl2023b} & ~ & 2023-11 & ~ & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        Vulpedia & \citeA{H.ZhangEtAl2023} & \href{https://github.com/ToolmanInside/vulpedia_demo}{url} & 2022-06 & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        ReDetect & \citeA{PanEtAl2021} & ~ & ~ & ~ & \ding{51} & \ding{51} & \ding{51} & ~ \\ 
        MEVD  & \citeA{L.ZhangEtAl2022a} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        Dynamit & \citeA{GhalebEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} \\ 
        Aroc & \citeA{LiangAndZhai2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        ConFuzzius & \citeA{LiuEtAl2023a} & \href{https://github.com/christoftorres/ConFuzzius}{url} & 2021-09 & Python & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        Cai \etal Framework & \citeA{VivarEtAl2021} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        SmartGraph & \citeA{JeonEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        S-BiGRU & \citeA{LiEtAl2022} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        GraphSA & \citeA{OtoniEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        Duan \etal Framework & \citeA{LongHeEtAl2023} & ~ & ~ & ~ & \ding{51} & \ding{51} & \ding{51} & ~ \\ 
        EDIT & \citeA{CaiEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        ASSBert & \citeA{DeSalveEtAl2024} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        GRATDet & \citeA{LiuEtAl2023b} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        Cao \etal Framework & \citeA{YangEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        AutoMESC & \citeA{LiEtAl2023} & \href{https://github.com/majdsoud/AutoMESC-Framework}{url} & 2023-09 & Python & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\ 
        AMAT & \citeA{SongEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} \\ 
        RNVulDet  & \citeA{Z.ZhangEtAl2022} & \href{https://github.com/Messi-Q/RNVulDet}{url} & 2023-07 & Python & \ding{51} & ~ & \ding{51} & \ding{51} \\ 
        SCVDIE & \citeA{XuEtAl2021} & \href{https://github.com/yzu-wjl/SCVDIE}{url} & 2022-05 & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        eTainter & \citeA{EshghieEtAl2021} & \href{https://github.com/DependableSystemsLab/eTainter}{url} & 2022-07 & Python & \ding{51} & ~ & \ding{51} & ~ \\ 
        Park & \citeA{OlsthoornEtAl2022} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & \ding{51} \\ 
        Achecker & \citeA{WangEtAl2022} & \href{https://github.com/DependableSystemsLab/Achecker}{url} & 2023-05 & Python & \ding{51} & ~ & \ding{51} & ~ \\ 
        SIGUARD & \citeA{HuangEtAl2021} & \href{https://github.com/Jiashuo-Zhang/Siguard}{url} & 2023-05 & Python & \ding{51} & ~ & \ding{51} & ~ \\ 
        SmartState & \citeA{QianEtAl2023c} & \href{https://github.com/InPlusLab/SmartState}{url} & 2023-07 & Python & \ding{51} & ~ & \ding{51} & ~ \\ 
        Teacher-Student Framework & \citeA{GhalebEtAl2022} & \href{https://github.com/Messi-Q/Cross-Modality-Bug-Detection}{url} & 2023-04 & Python & \ding{51} & ~ & \ding{51} & ~ \\ 
        SynTest-Solidity & \citeA{J.ZhangEtAl2023} & \href{https://github.com/syntest-framework/syntest-solidity}{url} & 2022-05 & TypeScript & ~ & \ding{51} & ~ & \ding{51} \\ 
        Elysium & \citeA{ZhengEtAl2022} & \href{https://github.com/christoftorres/Elysium}{url} & 2022-10 & JavaScript, Python & \ding{51} & ~ & \ding{51} & ~ \\ 
        Solicitous (2.0) & \citeA{NguyenEtAl2022} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        MagicMirror & \citeA{SoudEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        SMARTIAN & \citeA{YuEtAl2021} & \href{https://github.com/SoftSec-KAIST/Smartian}{url} & 2021-11 & F\# & \ding{51} & ~ & \ding{51} & \ding{51} \\ 
        CrossFuzz (Extends ConFuzzius) & \citeA{BarboniEtAl2022} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        Block-Gram & \citeA{HajiHosseinKhaniEtAl2024} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        EtherGIS & \citeA{LiuZEtAl2021} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        ESCORT & \citeA{dZaazaaAndElBakkali2023b} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        SVScanner & \citeA{FeiEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        Effuzz & \citeA{PasquaEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} \\ 
        SmartDagger & \citeA{AshizawaEtAl2021} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        ReVulDL & \citeA{TorresEtAl2022} & \href{https://github.com/toolstemp/Iacontract}{url} & ~ & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        ASGVulDetector & \citeA{SujeethaAndAkila2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        BASGVulDetector & \citeA{SujeethaAndAkila2023} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        TxMirror & \citeA{CaoEtAl2023b} & ~ & ~ & ~ & \ding{51} & ~ & ~ & \ding{51} \\ 
        TxSpector & ~ & \href{https://github.com/OSUSecLab/TxSpector}{url} & 2020-08 & Go & \ding{51} & ~ & ~ & \ding{51} \\ 
        SPCBIG-EC (SPCNN) & \citeA{LutzEtAl2021} & \href{https://github.com/wobulijie10086/SPCBIG-EC/tree/master/SPCBIG-EC}{url} & 2022-06 & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        CBGRU & \citeA{VaccaEtAl2021} & \href{https://github.com/xiaoaochen/CBGRU}{url} & 2022-05 & ~ & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        SmartBugs2.0 & \citeA{MaEtAl2023} & \href{https://github.com/smartbugs/smartbugs}{url} & 2021-11 & Python & \ding{51} & \ding{51} & \ding{51} & ~ \\ 
        GraBit & \citeA{HuEtAl2023b} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        PSCVFinder & \citeA{NguyenEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        HGAT & \citeA{L.ZhangEtAl2022c} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        EtherFuzz & \citeA{ChenEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} \\ 
        SoliTester & \citeA{BarboniEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} \\ 
        sFuzz2.0 & \citeA{BoseEtAl2021} & \href{https://github.com/duytai/sFuzz/tree/v2.0}{url} & 2023-02 & C++ & ~ & \ding{51} & ~ & \ding{51} \\ 
        HeEtAl2024 & \citeA{HeEtAl2024} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        TIPS & \citeA{SunEtAl2022a} & \href{https://github.com/CVbluecat/TIPS}{url} & 2023-09 & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        SCsVulLyzer & \citeA{YangEtAl2024} & \href{https://github.com/ahlashkari/SCsVulLyzer}{url} & 2024-02 & Python & ~ & \ding{51} & \ding{51} & ~ \\ 
        EtherSolve2.0 (Extends EtherSolve) & \citeA{JiamingYeEtAl2022} & \href{https://github.com/SeUniVr/EtherSolve}{url} & 2023-03 & Java & \ding{51} & ~ & \ding{51} & ~ \\ 
        MODNN & \citeA{Y.ZhangEtAl2022} & ~ & ~ & ~ & \ding{51} & \ding{51} & \ding{51} & ~ \\ 
        SuperDetector & \citeA{ZhuEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        SoliDetector & \citeA{L.ZhangEtAl2022b} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        SCcheck & \citeA{MahugnonAndJules2022} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        SESCon & \citeA{WangEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        Sailfish (built on Slither) & \citeA{diAngeloEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        MuIESC & \citeA{DaiEtAl2022} & \href{https://github.com/SmartcontractTest/MuIESC}{url} & 2022-02 & Python & ~ & \ding{51} & ~ & \ding{51} \\ 
        FSL-Detect & \citeA{Mazurek2021} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        EthVer & \citeA{Hong-NingEtAl2021} & \href{https://github.com/lukmaz/ethver}{url} & 2021-09 & Haskell & ~ & \ding{51} & \ding{51} & ~ \\ 
        Gas Gauge & \citeA{WuHEtAl2021} & \href{https://github.com/gasgauge/gasgauge.github.io}{url} & 2021-12 & Python & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        Pakala & \citeB{pakala2024} & \href{https://github.com/palkeo/pakala}{url} & 2018-12 & Python & \ding{51} & ~ & \ding{51} & ~ \\ 
        SolGuard (Extends Solhint) & \citeA{GuoEtAl2024} & ~ & 2021-08 & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        Ethlint  & ~ & \href{https://github.com/duaraghav8/Ethlint?tab=readme-ov-file}{url} & 2018-01 & JavaScript & ~ & \ding{51} & \ding{51} & ~ \\ 
        Solitor & \citeB{StegemanSolitor} & \href{https://github.com/LarsStegeman/EthereumRuntimeMonitoring}{url} & 2018-11 & Java & ~ & \ding{51} & ~ & \ding{51} \\ 
        SCSVM & \citeA{SunEtAl2022b} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        SCLMF & \citeA{SunEtAl2022b} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        Kaya & \citeB{WuEtAl2020} & \href{https://github.com/Ghands/Kaya}{url} & 2020-10 & JavaScript, Python & ~ & \ding{51} & ~ & \ding{51} \\ 
        ConFuzzius-BI & \citeA{LiaoEtAl2023} & \href{https://github.com/SmartcontractTest/ConFuzzius-BI/tree/main}{url} & 2022-12 & Python & ~ & \ding{51} & \ding{51} & \ding{51} \\ 
        Horus & \citeA{TorresEtAl2021b} & \href{https://github.com/christoftorres/Horus}{url} & 2021-01 & Python & ~ & \ding{51} & ~ & \ding{51} \\ 
        Ethchecker & \citeA{HanEtAl2024} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        Developer & \citeA{RongzeXuEtAl2022} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 
        DL4SC & \citeA{LiuEtAl2024} & \href{https://github.com/LaoSuanNaii/DL4SC}{url} & 2024-03 & Python & \ding{51} & ~ & \ding{51} & ~ \\ 
        HARDEN & \citeA{LakadawalaEtAl2024} & ~ & ~ & ~ & \ding{51} & ~ & \ding{51} & ~ \\ 
        Jie \etal Framework & \citeA{JieEtAl2023} & ~ & ~ & ~ & ~ & \ding{51} & \ding{51} & ~ \\ 

    \end{longtable}
}

==> tables/topten.tex <==
% \begin{table*}[h!]
% \centering
% \caption{Top 10 detected vulnerabilities.}
% \begin{tabular}{lr}
% \toprule
% \textbf{Vulnerability} & \textbf{Detection Tools} \\
% \midrule
% \rowcolor{gray!5}
% Reentrancy & 130 \\
% Timestamp dependency & 78 \\
% \rowcolor{gray!5}
% Integer overflow/underflow & 62 \\
% Unchecked low-level call/send return values & 51 \\
% \rowcolor{gray!5}
% Vulnerable delegatecall & 35 \\
% Authorization via transaction origin & 32 \\
% \rowcolor{gray!5}
% Unprotected selfdestruction & 31 \\
% Transaction-ordering dependency & 30 \\
% \rowcolor{gray!5}
% Greedy contract & 26 \\
% Block State Dependency & 15 \\
% \bottomrule
% \end{tabular}
% \end{table*}

% {\footnotesize
% \rowcolors{2}{gray!5}{white}  % Start alternating colors from row 2
% \begin{longtable}{lr}
%     \caption{Top 10 detected vulnerabilities.} 
%     \label{tab:topten}\\
%     \toprule
%     \textbf{Vulnerability} & \textbf{Detection Tools} \\ 
%     \midrule
%     Reentrancy & 130 \\
%     Timestamp dependency & 78 \\
%     Integer overflow/underflow & 62 \\
%     Unchecked low-level call/send return values & 51 \\
%     Vulnerable delegatecall & 35 \\
%     Authorization via transaction origin & 32 \\
%     Unprotected selfdestruction & 31 \\
%     Transaction-ordering dependency & 30 \\
%     Greedy contract & 26 \\
%     Block State Dependency & 15 \\
%     \bottomrule
% \end{longtable}
% }

\begin{table}[!h]
    \centering
    \scriptsize
    \caption{Top 10 detected vulnerabilities.}
    \label{tab:topten}
    \rowcolors{2}{gray!5}{white}
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{lr}
        \toprule
        \textbf{Vulnerability} & \textbf{Detection Tools} \\
        \midrule
        Reentrancy & 130 \\
        Timestamp dependency & 78 \\
        Integer overflow/underflow & 62 \\
        Unchecked low-level call/send return values & 51 \\
        Vulnerable delegatecall & 35 \\
        Authorization via transaction origin & 32 \\
        Unprotected selfdestruction & 31 \\
        Transaction-ordering dependency & 30 \\
        Greedy contract & 26 \\
        Block State Dependency & 15 \\
        \bottomrule
    \end{tabular}
    % }
\end{table}

